Deep Reinforcement Learning Versus Evolution Strategies: A Comparative Survey

Deep Reinforcement Learning (DRL) and Evolution Strategies (ESs) have surpassed human-level control in many sequential decision-making problems, yet many open challenges still exist. To get insights into the strengths and weaknesses of DRL versus ESs, an analysis of their respective capabilities and limitations is provided. After presenting their fundamental concepts and algorithms, a comparison is provided on key aspects such as scalability, exploration, adaptation to dynamic environments, and multi-agent learning. Then, the benefits of hybrid algorithms that combine concepts from DRL and ESs are highlighted. Finally, to have an indication about how they compare in real-world applications, a survey of the literature for the set of applications they support is provided.

==> sections/draft/DRL.tex <==
Throughout this section, we will introduce the concept of Reinforcement Learning: its basic elements, concepts and terminology, a high level explanation of how it works and some of the underlying algorithms.

\subsection{Background}
Reinforcement Learning  is a branch of machine learning in which an agent learns by trial and error from interacting with an environment. The algorithm (an agent) evaluates a current situation (state), takes an action, and receives feedback (reward) from the environment after each act. Positive feedback is a reward , and negative feedback is punishment for making a mistake, formalizing the idea that rewarding or punishing an agent for its behavior makes it more likely to repeat or forego that behavior in the future. In Reinforcement learning, the goal of the agent is therefore to maximize its cumulative reward. \\

The basic elements of RL include:
\begin{itemize}
  \item Agent: the learner and the decision maker
  \item Environment: where the agent learns and decides what actions to perform
  \item Action: a set of actions which the agent can perform
  \item State: the state of the agent in the environment.
  \item Reward: for each action selected by the agent the environment provides a reward. Usually a scalar value
  \item Policy: the decision-making function (control strategy) of the agent, which represents a mapping from situations to actions. It can be deterministic or stochastic. In deep RL, we deal with parameterized policies: policies whose outputs are computable functions that depend on a set of parameters (eg the weights and biases of a neural network) which we can adjust to change the behavior via some optimization algorithm. We often denote the parameters of such a policy by $\theta$
  \item Deterministic Policy: Is a function from the set of states of the environment, S, to the set of actions, A. 
  \item Stochastic Policy: is often represented as a family of conditional probability distributions, $\pi_s(A|S)$, from the set of states, S, to the set of actions A. A probability distribution is a function that assigns a probability for each event (in this case, the events are actions in certain states) and such that the sum of all the probabilities is 1
  \item Value function: mapping from states to real numbers, where the value of a state represents the long-term reward achieved starting from that state, and executing a particular policy
  \item Function approximator: refers to the problem of inducing a function from training examples. Standard approximators include decision trees, neural networks, and nearest-neighbor methods
  \item Markov decision process (MDP): A probabilistic model of a sequential decision problem, where states can be perceived exactly, and the current state and action selected determine a probability distribution on future states. Essentially, the outcome of applying an action to a state depends only on the current action and state (and not on preceding actions or states).
  \item Dynamic programming (DP): is a class of solution methods for solving sequential decision problems with a compositional cost structure. Richard Bellman was one of the principal founders of this approach
  \item Monte Carlo methods: A class of methods for learning of value functions, which estimates the value of a state by running many trials starting at that state, then averages the total rewards received on those trials
  \item Temporal Difference (TD) algorithms: A class of learning methods, based on the idea of comparing temporally successive predictions. Possibly the single most fundamental idea in all of reinforcement learning
  \item Model: The agent’s view of the environment, which maps state-action pairs to probability distributions over states. Note that not every reinforcement learning agent uses a model of its environment
  \item Exploration: you search over the whole sample space (exploring the sample space)
  \item Exploitation: exploiting the promising areas found when you did the exploration
\end{itemize}

\noindent A reinforcement learning problem is therefore usually set up as a Markov Decision Process (MDP). In its simplest form, an MDP consist of an agent, a set of states, a set of actions, a state-transition model and a reward function. The agent act in the environment by taking actions which allow him to transition between states. The state-transition model describes for every action the probability of ending up in each of the states. The reward function specifies the immediate reward obtained after transitioning from a state to another state. As many application involve incomplete information about the environment the problem is often formulated as a partially observable MDP (POMDP). A POMDP extends the definition of an MDP with a set of observations and an observation probability distribution. After every transition an agent receives an observation. The probability of receiving this observation depends on the current state and the action just taken as specified by the observation probability distribution. The agent's ultimate goal is to maximize the long term cumulative rewards.\\

\noindent There are two main strategies to solve DMP problems, model-based, and model-free.  Despite their data efficiency, model-based methods (e.g., dynamic programming methods) require full knowledge of the environment to plan an optimal solution. Therefore, they face difficulty tackling complex problems with large and unknown environments. Model-free methods, on the other hand, do not require full knowledge of the environment and aim at learning a policy ---a function that maps a given state to an specific action--- to maximize the agent's long term cumulative reward~\cite{ding2020introduction}. The final policy which maximizes the long-term reward is called an optimal policy. \\

\noindent Based on which metric is being used to learn the optimal policy model-free RL methods can be subdivided into two main approaches:
\begin{itemize}
\item \textit{Value-based optimization algorithms} learn the optimal policy via the value of the action taken in a state (symbolically defined as $Q(s,a)$). Examples of such algorithms are value iteration~\cite{valueiter}, Q-learning, DQN~\cite{DQN}, and SARSA~\cite{SARSA}.

\item \textit{Policy-based optimization algorithms} learn the optimal policy via the value of the state. Examples of such algorithms are policy iteration~\cite{policyiter}, policy gradient~\cite{policygradient} and REINFORCE~\cite{reinforce}. 
\end{itemize}

\noindent Both of these approaches have their advantages. Value-based algorithms are sample efficient and steady while policy-based methods in comparison show better performance in continuous and stochastic environments. \\

Machine learning is able to at least partially overcome the problem of high-dimensionality. Deep RL in particular, which was first introduced in 2015 by \citet{Mnih2015} has proven to be adequate for handling highly dimensional input data. \\

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/drlhistory.png}
    \caption{Emergence of deep RL through different essential milestones, by \citet{Nguyen2020_challenges}}
    \label{drl_graph}
\end{figure}

\noindent Before diving into the different Deep RL applications and their associated research papers, we will provide below a brief background on the emergence of Deep RL and how Deep RL works. Figure \ref{drl_graph} by \citet{Nguyen2020_challenges} outlines the chronological milestones in the history of machine learning leading up to the Deep RL of today. Notably, in 1989 \citet{Watkins1992} combined optimal control theory including the \textit{Bellman equation} and \textit{Markov decision process} in conjunction with \textit{temporal-difference learning} to form the well-known \textit{Q-learning} which found many real-world applications. However, a severe limitation of Q-learning as conceived by Watkins and Dayan is the inability to deal with high-dimensional problems as the number of calculations increases drastically with the number of inputs, beyond the computational capabilities of conventional computers. In 2015, Mnih et al. \cite{Mnih2015} published their revolutionary work for the first time combining deep learning with RL to partially overcome the problem of hyperdimensionality. \\

Deep Reinforcement Learning (DRL), a very fast-moving field, is the combination of Reinforcement Learning and Deep Learning and it is also the most trending type of Machine Learning at this moment because it is being able to solve a wide range of complex decision-making tasks that were previously out of reach for a machine to solve real-world problems with human-like intelligence.

Deep RL combines the ability to process highly-dimensional input using a deep neural network with the flexibility of reinforcement learning to produce a highly scalable and adaptive system. After training, the resulting model can be copied and distributed over any number of agents. 

\begin{figure}[htbp]
\centerline{\includegraphics[width=\columnwidth]{RL.pdf}}
\caption{Deep Reinforcement learning landscape. This figure showcases the overall DRL architecture focused on the agent and the environment}
\label{fig2}
\end{figure}

\subsection{Common algorithms}
This  section will go over the main Reinforcement and Deep Reinforcement Learning algorithms, covering them at a high level.\\
Q-Learning \cite{mnih2013playing} is an off-policy, model-free RL algorithm. It is a primitive form of Reinforcement Learning which leverages Q-values (action values) to iteratively optimize the behavior of the learning agent. Three main steps are involved in Q-Learning:
\begin{itemize}
  \item Q-Values : Q-values are characterized by states and actions. $Q(S, A)$ is an measure of the total expected reward assuming the Agent is in state $S$ and performs action $A$. This estimation of $Q(S, A)$ will be iteratively computed using TD- Update defined below.
  \item Rewards and Episodes: As seen in Figure \ref{fig2}, as part of the overall DRL landscape, an agent starts from a start state, makes a number of transitions from its current state to a next state based on an a specific action and on the environment. At every iteration, the agent from a state performs an action, and is rewarded from the environment, before moving to another state. An agent hits a terminating state whenever there are no further transition possible, and the episode is said to be completed. \remark{Not all DRL problems can be regarded as episodic problems. What about problems with continuous states?}
  \item Temporal Difference based on the formula: \\
  $Q(s_t,a_t)\leftarrow Q(s_t,a_t)+\alpha(r_(t+1)+\gamma max_a Q(s_(t+1),a_(t+1))-Q(s_t,a_t))$
\end{itemize}
SARSA algorithm is a slight variation of the popular Q-Learning algorithm. It is an on-policy, model-free RL algorithm. The difference with Q-learning is visible in the Temporal Difference formula :\\ 
$Q(s_t,a_t)\leftarrow Q(s_t,a_t)+\alpha(r_(t+1)+\gamma Q(s_(t+1),a_(t+1))-Q(s_t,a_t))$

\remark{So what are the principles behind DRL?}

==> sections/draft/DRL_previous.tex <==
\subsection{Main principles behind Deep Reinforcement learning}

During the last decade the developments in machine learning have drastically impacted and lead to new perspectives in many fields, including that of multi-agent systems. 
Machine learning is able to at least partially overcome the problem of high-dimensionality. Deep RL in particular, which was first introduced in 2015 by \citet{Mnih2015} has proven to be adequate for handling highly dimensional input data. \\
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/drlhistory.png}
    \caption{Emergence of deep RL through different essential milestones, by \citet{Nguyen2020_challenges}}
    \label{drl_graph}
\end{figure}
\noindent Before diving into the different Deep RL applications and their associated research papers this section will provide a brief background on the emergence of Deep RL and how Deep RL works. Figure \ref{drl_graph} by \citet{Nguyen2020_challenges} outlines the chronological milestones in the history of machine learning leading up to the Deep RL of today. Notably, in 1989 \citet{Watkins1992} combined optimal control theory including the \textit{Bellman equation} and \textit{Markov decision process} in conjunction with \textit{temporal-difference learning} to form the well-known \textit{Q-learning} which found many real-world applications. However, a severe limitation of Q-learning as conceived by Watkins and Dayan is the inability to deal with high-dimensional problems as the number of calculations increases drastically with the number of inputs, beyond the computational capabilities of conventional computers. In 2015, Mnih et al. \cite{Mnih2015} published their revolutionary work for the first time combining deep learning with RL to partially overcome the problem of hyperdimensionality. \\

\noindent A reinforcement learning problem is usually set up as a Markov Decision Process (MDP). In its simplest form, an MDP consist of an agent, a set of states, a set of actions, a state-transition model and a reward function. The agent act in the environment by taking actions which allow him to transition between states. The state-transition model describes for every action the probability of ending up in each of the states. The reward function specifies the immediate reward obtained after transitioning from a state to another state. As many application involve incomplete information about the environment the problem is often formulated as a partially observable MDP (POMDP). A POMDP extends the definition of an MDP with a set of observations and an observation probability distribution. After every transition the robot receives an observation. The probability of receiving this observation depends on the current state and the action just taken as specified by the observation probability distribution. The agent's ultimate goal is to maximize the long term cumulative rewards.\\

\noindent There are two main strategies to solve DMP problems, model-based, and model-free.  Despite their data efficiency, model-based methods (e.g., dynamic programming methods) require full knowledge of the environment to plan an optimal solution. Therefore, they face difficulty tackling complex problems with large and unknown environments. Model-free methods, on the other hand, do not require full knowledge of the environment and aim at learning a policy ---a function that maps a given state to an specific action--- to maximize the agent's long term cumulative reward~\cite{ding2020introduction}. The final policy which maximizes the long-term reward is called an optimal policy. \\

\noindent Based on which metric is being used to learn the optimal policy model-free RL methods can be subdivided into two main approaches:
\begin{itemize}
\item \textit{Value-based optimization algorithms} learn the optimal policy via the value of the action taken in a state (symbolically defined as $Q(s,a)$). Examples of such algorithms are value iteration~\cite{valueiter}, Q-learning, DQN~\cite{DQN}, and SARSA~\cite{SARSA}.

\item \textit{Policy-based optimization algorithms} learn the optimal policy via the value of the state. Examples of such algorithms are policy iteration~\cite{policyiter}, policy gradient~\cite{policygradient} and REINFORCE~\cite{reinforce}. 
\end{itemize}

\noindent Both of these approaches have their advantages. Value-based algorithms are sample efficient and steady while policy-based methods in comparison show better performance in continuous and stochastic environments. \\

Deep RL combines the ability to process highly-dimensional input using a deep neural network with the flexibility of reinforcement learning to produce a highly scalable and adaptive system. After training, the resulting model can be copied and distributed over any number of agents. 

\begin{figure}[htbp]
\centerline{\includegraphics[width=\columnwidth]{RL.pdf}}
\caption{Deep Reinforcement learning landscape. This figure showcases the overall DRL architecture focused on the agent and the environment}
\label{fig2}
\end{figure}

\subsection{Common algorithms}
This section will go over the main Reinforcement and Deep Reinforcement Learning algorithms, covering them at a high level.\\
Q-Learning \cite{mnih2013playing} is an off-policy, model-free RL algorithm. It is a primitive form of Reinforcement Learning which leverages Q-values (action values) to iteratively optimize the behavior of the learning agent. Three main steps are involved in Q-Learning:
\begin{itemize}
  \item Q-Values : Q-values are characterized by states and actions. $Q(S, A)$ is an measure of the total expected reward assuming the Agent is in state $S$ and performs action $A$. This estimation of $Q(S, A)$ will be iteratively computed using TD- Update defined below.
  \item Rewards and Episodes: As seen in Figure \ref{fig2}, as part of the overall DRL landscape, an agent starts from a start state, makes a number of transitions from its current state to a next state based on an a specific action and on the environment. At every iteration, the agent from a state performs an action, and is rewarded from the environment, before moving to another state. An agent hits a terminating state whenever there are no further transition possible, and the episode is said to be completed. \remark{Not all DRL problems can be regarded as episodic problems. What about problems with continuous states?}
  \item Temporal Difference based on the formula: \\
  $Q(s_t,a_t)\leftarrow Q(s_t,a_t)+\alpha(r_(t+1)+\gamma max_a Q(s_(t+1),a_(t+1))-Q(s_t,a_t))$
\end{itemize}
SARSA algorithm is a slight variation of the popular Q-Learning algorithm. It is an on-policy, model-free RL algorithm. The difference with Q-learning is visible in the Temporal Difference formula :\\ 
$Q(s_t,a_t)\leftarrow Q(s_t,a_t)+\alpha(r_(t+1)+\gamma Q(s_(t+1),a_(t+1))-Q(s_t,a_t))$

\remark{So what are the principles behind DRL?}

==> sections/draft/RLvsES.tex <==
% With the advances in the field of Deep Reinforcement Learning, methods are becoming extremely complicated and less robust to changes in the hyperparameters or random seeds. Simplified model-free RL methods are thus being increasingly looked into for solving standard computation.
% A recurring issue in Reinforcement Learning tasks is to find the policies to be applied on the dynamic system in order to optimize future reward by maximizing it. As previously mentioned, the agent should thus follow specific policies which will identify the next action to take based on the current state. Two main approaches are identified in a model free setting as shown in the Figure \ref{fig1}: Value based and policy based optimization.
% \begin{figure}[htbp]
% \centerline{\includegraphics[width=3.3in]{RL_freemodel.pdf}}
% \caption{Model free Reinforcement Learning overview}
% \label{fig1}
% \end{figure}

% \begin{figure*}[htbp]
% \centerline{\includegraphics[width=8in]{images/summary.png}}
% \caption{General timeline for ES and DRL}
% \label{fig_summary}
% \end{figure*}

%  While a value based optimization attempts to find a policy that maximizes the return by maintaining a set of estimates of expected returns for some policy, Direct policy search methods addresses this task by directly learning parameters of a function explicitly representing the policy. \cite{Verena2008}
% \noindent The rest of this section will go over the main advancements in the Evolution Strategies' field as they compare to Deep Reinforcement Learning. Each of the ES algorithms previously defined: CMA-ES, NES and OpenAI ES, was thus identified in the literature as a viable alternative for Deep Reinforcement Learning algorithms, and the details of such implementation and experimentation results will be discussed thereafter. Moreover some of the improvements identified for  Evolution Strategies will be discussed in further details, before trying to identify the most viable approach. Finally a comparison from the applications' and usage point of view will be performed.

% \subsection{Evolution Strategies as a solution}% Identifed Solutions

% \begin{table*}[htbp]
% \caption{Selected algorithms from the Evolution Strategies family}
% \begin{center}
% \label{t1}
% \begin{tabular}{p{0.22\linewidth} | p{0.22\linewidth} | p{0.40\linewidth}| p{0.10\linewidth}}
%  \hline 
%  Algorithm , references & Author & Short description & Year \\
%  \hline\hline  
%   OpenAI Evolution Strategy (OpenAI-ES) & Salimans et al. & The authors proposed an Evolution Strategy implementation scalable over a thousand parallel workers, and highlight several advantages of ES as a black box optimization technique & 2017 \\ 
%  \hline
%   OpenAI Evolution Strategy (OpenAI-ES) & Zhang et al. & Explores the relationship between ES and SGD by comparing the approximate gradient computed by ES with the exact gradient computed by SGD in MNIST under different conditions & 2017 \\ 
%  \hline
%  Canonical ES & Chrabaszcz et al. & The authors proposed an Evolution Strategy implementation scalable over a thousand parallel workers, and highlight several advantages of ES as a black box optimization technique & 2018 \\
%  \hline
%   Restart-based rank-1 evolution strategy (R-R1-ES) & Chen et al. & The authors proposed R-R1-ES, a simplified CMA-ES for large scale black-box optimization, and involves the procedures of adapting the mutation strength, updating the distribution and the principal search direction, and escaping local optima & 2019 \\ 
%  \hline
%  Instance weighted incremental evolution strategy (IW-IES) & Liu et al. & The authors develop an algorithm called Trust Region Evolution Strategies (TRES), which leads to better performance than ES algorithm by ensuring more efficient using of sampled data & 2019 \\ 
%  \hline
%  Trust Region Evolution Strategies (TRES) & Wang et al. & The authors formulate an incremental learning procedure that uses natural evolution strategies (NES) to update the parameters of a policy network for RL in dynamic environments & 2020 \\ 
%  \hline
%  ES-MAML & Song et al. & The authors introduce ES-MAML, a new framework for solving the model agnostic meta learning (MAML) problem based on Evolution Strategies (ES) & 2020 \\ 
%  \hline
%  ES-MAML & Song et al. & The authors present a new meta-learning method that allows robots to quickly adapt to changes in dynamics & 2020 \\ 
%  \hline
% \end{tabular}
% \label{tab1}
% \end{center}
% \end{table*}

% As seen in Figure \ref{fig1}, policy search methods usually use either gradient-based or gradient-free optimization, and both can successfully train neural networks to encode policies.Gradient-based optimization enables relatively efficient learning, it is still however extremely sensitive to hyperparameter choices and does not have good convergence properties \cite{Bruin2020IFAC}. As for gradient-free optimization such as Evolution Strategies, the latter can adequately cater for low-dimensional parameter spaces but faces some difficulties when applied to large networks with a large number of parameters. Seeing how Gradient-based optimization is considered to be the de facto methods for optimizing neural networks with millions of parameters, Evolution Strategies resurfaced lately and their performance was tested accordingly. \\ 
% \noindent We will thus discuss below how recent results have shown that various Evolution Strategy algorithms or variations on the latter can rival the performance of reinforcement learning (RL) on a set of challenging deep RL problems.\\

% \subsubsection{Parallel scaling across many workers}\hspace*{\fill} \\

% The OpenAI Evolutionary Strategy \cite{salimans2017evolution} (OpenAI-ES) introduced several contributions for improving the training and performance and be able to compete with state-of-the-art RL algorithms, all the while renewing interest in ES methods. Additionally, the simplicity of ES made it suitable for parallel scaling across many workers and makes it scalable and efficient to use on distributed hardware \cite{salimans2017evolution}. Moreover, RL methods such as A3C need to communicate gradients back and forth between workers and a parameter server, while OpenAI-ES only requires fitness scores and high-level parameter distribution information to be communicated. 
% %All of this comes at a cost however: the cost of treating the network being optimized as a black-box.
% Another contribution by Salimans et al. \cite{salimans2017evolution} is the usage of virtual batch normalization \cite{salimans2016improved} to make the network output more sensitive to the noise in the parameter space. Salimans et al. applied OpenAI-ES to MuJoCo (continuous robotic control, eg  walking/hopping/swimming) tasks and several Atari games. OpenAI-ES was able to solve the MuJoCo tasks and performed competitively on the Atari games \cite{salimans2017evolution}, showcasing that OpenAI-ES can compete with some RL algorithms in terms of performance on the hardest problems solvable today, and is close in terms of data efficiency, while taking less wallclock time to train. Moreover,  as noted by the authors, this approach decreases the probability of falling into local optima early and lowers the influence of outliers.

% These results from Salimans et al. \cite{salimans2017evolution} provoked surprise as ES was shown to rival the performance of stochastic gradient descent (SGD)-based deep RL methods with large neural networks. Zhang et al. \cite{zhang2017relationship} thus investigated the relationship between the OpenAI-ES and the stochastic gradient descent method by conducting several MNIST-based experiments, aiming to give additional insights into the behaviors of ES, to better understand how and when OpenAI-ES can rival SGD-based RL algorithms. Zhang et al. \cite{zhang2017relationship} then clearly went over the work of Salimans et al. \cite{salimans2017evolution} in an effort to list the benefits provided by it, and achieved 99\% accuracy on MNIST, a number higher than any previously published result for any evolutionary method.\\

% \subsubsection{Meta-Learning with Evolution Strategies}\hspace*{\fill} \\

% \subsection {Improving on Evolution Strategies}
% Following OpenAI’s work \cite{salimans2017evolution}, several researchers attempted to improve the performance of Evolutionary Strategies. Conti et al. \cite{conti2018improving} thus introduced novelty search (NS) and quality diversity (QD), and formed two algorithms (called NS-ES and NSR-ES, respectively). The algorithms presented can effectively avoid local optima confronted by Evolution Strategies. \citet{conti2018improving} showcased that novelty search (NS) and quality diversity (QD) algorithms, can be used in tandem with ES to improve its performance on sparse or deceptive deep RL tasks, while retaining scalability.\\
% Another improvement was the introduction of Progressive Episode Lengths (PEL) \cite{ijcai2019} into the canonical ES implementation of \citet{chrabaszcz2018basics}. The main objective of PEL is to allow the agent to play short and easy tasks with limited lengths, and then use the gained knowledge to further solve long and hard tasks with progressive lengths. This allows the agent to perform many function evaluations and find a good solution for short time horizons before adapting the strategy to tackle larger time horizons. The PEL approach is based on incremental learning, where an agent utilizes the capabilities obtained in limited games for an entire episodic run. The goal of this approach is thus to achieve more stable and faster optimization process by focusing on simpler and shorter tasks first. When integrating it with canonical ES, the latter is able to optimize by only playing a portion of a game, transferring the abilities obtained in a short game to a longer one. 

% \begin{table*}[htbp]
% \caption{Selected algorithms for improving Evolution Strategies}
% \begin{center}
% \label{t1}
% \begin{tabular}{p{0.22\linewidth} | p{0.22\linewidth} | p{0.40\linewidth}| p{0.10\linewidth}}
%  \hline 
%  Algorithm , references & Author & Short description & Year \\
%  \hline\hline  
%   Novelty Search Evolution Strategies (NS-ES) and Quality Diversity Evolution Strategies (QD-ES) & Conti et al. & The authors show that algorithms that have been invented to promote directed exploration in small-scale evolved neural networks via populations of exploring agents, specifically novelty search (NS) and quality diversity (QD) algorithms can be hybridized with ES to improve its performance on sparse or deceptive deep RL tasks, while retaining scalability & 2018 \\ 
%  \hline
%   Structured Evolution with Compact Architectures for Scalable Policy Optimization & Choromanski et al. & The authors present a new method of blackbox optimization via gradient approximation with the use of structured random orthogonal matrices. The algorithm can be successfully applied to learn better quality compact policies than those using standard gradient estimation techniques & 2018 \\ 
%  \hline
%   Progressive Episode Lengths Evolution Strategies (PEL-ES) & Fuks et al. & The authors introduce Progressive Episode Lengths (PEL) as a new technique and incorporate it with ES. The main objective is to allow the agent to play short and easy tasks with limited lengths, and then use the gained knowledge to further solve long and hard tasks with progressive lengths & 2019 \\ 
%  \hline
%   Flexible search distributions with GNNs (GNN-ES) & Faury et al. & This paper investigates the potential benefits of using highly flexible search distributions in classical ES algorithms and introduce a new training algorithm that leverages their expressiveness to accelerate the ES procedure & 2019 \\ 
%  \hline
%   Guided Evolutionary Strategies & Maheswaranathan et al. & The authors propose
%   Guided Evolutionary Strategies, a method for optimally using surrogate gradient directions along with random search & 2019 \\ 
%  \hline
%   ASEBO & Choromanski et al. & The authors propose
%   ASEBO, an algorithm that adapts to the geometry of the function and learns optimal
%   sets of sensing directions, which are used to probe it, on-the-fly, leading to more sample-efficient blackbox optimization than state-of-the-art algorithms & 2019 \\ 
%  \hline
%   Robust Blackbox Optimization (RBO) & Choromanski et al. & The authors propose a new class of algorithms, called Robust Blackbox Optimization (RBO) able to train policies effectively even in the rpesence of adverserial noise & 2019 \\ 
%  \hline
%   Variance reduction technique for ES & Tang et al. & The authors propose a new method for improving accuracy of the ES algorithms, that as opposed to
%   recent approaches utilizing only Monte Carlo structure of the gradient estimator, takes advantage of the underlying Markov decision process (mdp) structure to reduce the variance & 2020 \\ 
%  \hline
% \end{tabular}
% \label{tab1}
% \end{center}
% \end{table*}

% %This section needs to be elaborated upon
% \subsection {Is there a "one-size-fit-all" strategy}
% As previously mentioned, both methods have several advantages and weaknesses which will depend on their actual utilization. The distinguishing properties of each of these two types of algorithms thus come into play when having to choose the most suitable approach.\\ 
% When comparing these methods, the term sample efficiency is mainly used in the literature. Based on Sigaud et al. \cite{sigaud2019policy}, sample efficiency is critical for robotics systems, and covers three main parts:
% \begin{itemize}
%   \item "Data efficiency, i.e. extracting more information from available data" \cite{sigaud2019policy}
%   \item "Sample choice, i.e. obtaining data in which more information is available" \cite{sigaud2019policy}
%   \item "Sample reuse, i.e. improving a policy several times by using the same samples more than once through experience replay" \cite{sigaud2019policy}
% \end{itemize}
% From one end, Evolutionary Strategies are significantly less sample efficient than Deep Reinforcement learning methods as they learn from complete episodes, whereas Deep Reinforcement learning methods uses elementary steps of the system as samples, and thus exploit more information \cite{sigaud2019policy}. 
% Understanding how and when ES can rival SGD-based RL algorithms is thus critical. When using Reinforcement learning, learning often requires multiple trials or rollouts as when the gradient method is used, finding the optimized performance may be subject to environmental noise which worsens the adequacy of the gradient, and creates the risk of converging towards a local optima when greedily maximizing local reward. Moreover, these rollouts cannot be done in parallel as in ES since SGD methods require sending the gradient vectors of potentially millions of dimensions between the different cores. As previously mentioned, ES however offers a parallelism advantage as the random seeds used for the rollouts are the ones shared over the different cores. ES also seeks out more robust areas of the search space.\\
% An aspect that is sometimes overlooked as well is the analysis of the reward function based on the method used. Functions optimized for reinforcement learning may not necessarily be effective for Evolutionary Strategies and vice versa. The performance can thus be improved drastically when choosing the right reward function. The latter means that several of the comparisons made as of now were often biased towards one approach or the other \cite{pagliuca2020efficacy}.

% %This section needs yet to be filled
% \subsection {Comparison from an application point of view}

% \begin{table*}[htbp]
% \caption{Selected algorithms for improving Evolution Strategies}
% \begin{center}
% \label{t1}
% \begin{tabular}{p{0.22\linewidth} | p{0.22\linewidth} | p{0.40\linewidth}| p{0.10\linewidth}}
%  \hline 
%  Algorithm , references & Author & Short description & Year \\
%  \hline\hline  
%   Real-Time Task Assignment Approach Leveraging Reinforcement Learning with Evolution Strategies for Long-Term Latency Minimization in Fog Computing \cite{Mai_2018} & Mai et al. & The authors propose a reinforcement learning approach that utilizes the evolution strategies for real-time task assignment among fog servers to minimize the total computation latency during a long-term period. & 2020 \\ 
%  \hline
%   Smart usage of multiple RAT in IoT-oriented 5G networks: A Reinforcement Learning approach \cite{Sandoval_2018} & Sandoval et al. & The authors formulated the problem of deciding which Radio Access Technologies (RATs) should an IoT node employ when reporting events using Reinforcement Learning and Evolution Strategies. These transmission policies maximize a predefined reward closely related to classical throughput while keeping power consumption and operational costs below a certain limit & 2018 \\ 
%  \hline
%   A Reinforcement Learning-Based Framework for the Exploitation of Multiple RATs in the IoT \cite{8817919} & Sandoval et al. & The authors made use of Reinforcement Learning to allow IoT nodes to learn from previous real world data in order to derive optimal RAT-selection policies implemented as Artificial Neural Networks (ANN), maximize a predefined reward closely related to classic throughput, while maintaining power consumption and operational costs below a certain limit & 2019 \\ 
%  \hline
%  Fast converging evolutionary strategy for multi-constraint QoS routing in computer networks using new decoding mechanisms  \cite{Shahhoseini_2017} & Shahhoseini et al. & The authors propose a novel multi-constraints QoS routing algorithm based on Evolutionary Strategies (ES) & 2017 \\ 
%  \hline
%  An evolution strategy based approach for cover scheduling problem in wireless sensor networks  \cite{Srivastava2020AnES} & Srivastava et al. & This paper presents a (1 + 1)-evolution strategy based approach to address the Cover scheduling problem in wireless sensor networks (WSN-CSP) & 2019 \\ 
%  \hline
%  An analytical model to minimize the latency in healthcare internet-of-things in fog computing environment  \cite{Shukla} & Shukla et al. & XX & 2019 \\ 
%  \hline
% \end{tabular}
% \label{tab1}
% \end{center}
% \end{table*}


==> sections/draft/comparison_draft.tex <==
\subsection{General comparison} %\remark{WIP}
As previously mentioned, Evolution Strategies are as of late being be considered as alternatives to conventional Reinforcement Learning using back-propagation for training a deep neural network.
Throughout this section, we will compare both methods. We will first go through the challenges faced by each and the advantages they may bring when implemented over the other method.  

\subsubsection{Advantages and Weaknesses of Reinforcement learning}
Throughout this section We will go through the main advantages and disadvantages of DRL. Focusing on the advantages it brings to the table as  compared to ES(why would it be chosen over the latter, etc.).\\
DRL is sample efficient, since it learns from every step of an episode \cite{sigaud2019policy}. Off-policy deep RL algorithms can use a replay buffer to exploit the same samples as many times as useful, greatly improving sample efficiency \cite{pourchot2019cemrl}. Deep reinforcement learning makes it possible to train control policies that map high dimensional observations to actions \cite{Bruin2020IFAC}.\\
However, The gradient information of the objective functions can be unavailable at times. First-order optimization methods such as gradient descent may fail. Poor stability as it is sensitive to hyperparameters \cite{Bruin2020IFAC}. DRL uses gradient-based optimization techniques do not have good convergence properties \cite{Bruin2020IFAC}. In the context of robotics, sample efficiency is a key concern. There are three aspects to sample efficiency: (1) data efficiency, i.e. extracting more information from available data (definition taken from (Deisenroth and Rasmussen, 2011)), (2) sample choice, i.e. obtaining data in which more information is available and (3) sample reuse, i.e. improving a policy several times by using the same samples more than once through experience replay. \cite {sigaud2019policy}
Moreover, Deep Reinforcement learning typically suffer from three core difficulties: temporal credit assignment with sparse rewards, lack of effective exploration, and . Collectively, these challenges severely limit the applicability of these approaches to real-world problems \cite{Khadka2018}.
First, associating actions with returns when a reward is sparse (only observed after a series of actions) is difficult. This is a common occurrence in most real world domains and is often referred to as the temporal credit assignment problem [56]. Temporal Difference methods in RL use bootstrapping to address this issue but often struggle when the time horizons are long and the reward is sparse. Multi-step returns address this issue but are mostly effective in on-policy scenarios [12, 47, 48]. Offpolicy multi-step learning [36, 50] have been demonstrated to be stable in recent works but require
complementary correction mechanisms like importance sampling, Retrace [39, 61] and V-trace [16] which can be computationally expensive and limiting.\\
Secondly, RL relies on exploration to find good policies and avoid converging prematurely to local optima. Effective exploration remains a key challenge for DRL operating on high dimensional action and state spaces [43]. Many methods have been proposed to address this issue ranging from count-based exploration [40, 57], intrinsic motivation [5], curiosity [42] and variational information maximization [28]. A separate class of techniques emphasize exploration by adding noise directly to the parameter space of agents [22, 43]. However, each of these techniques either rely on complex supplementary structures or introduce sensitive parameters that are task-specific. A general strategy for exploration that is applicable across domains and learning algorithms is an active area of research.\\
Finally, DRL methods are notoriously sensitive to the choice of their hyperparamaters [27, 29] and often have brittle convergence properties [26]. This is particularly true for off-policy DRL that utilize a replay buffer to store and reuse past experiences [6]. The replay buffer is a vital component in enabling sample-efficient learning but pairing it with a deep non-linear function approximator leads to extremely brittle convergence properties [15, 26].

\subsubsection{Advantages and Weaknesses of Evolution Strategies}
ES usually outperform gradient-based approaches in the presence of noise and on multimodal objective functions (especially if the local optima have only small basins of attraction) \cite{Verena2008}.\\
Since ES only needs to communicate scalar returns of complete episodes, it is highly parallelizable and enables near-linear speedups in runtime as a function of CPUs. ES uses a fitness metric that consolidates returns across an entire episode, making it invariant to sparse or deceptive rewards with arbitrarily long time horizons. The population-based evolutionary search provides diverse exploration, particularly when combined with explicit diversity maintenance techniques. Moreover, the redundancy inherent in a population also facilitates
robustness and stable convergence properties, especially when incorporated with elitism \cite{wang2020instance}.\\
Evolution Strategies (ES) (Salimans et al. 2017) has been risen to be a viable alternative to popular MDP-based RL techniques. As comparable to state-of-the-art policy gradient methods, ES has demonstrated its success in training policies on a variety of simulated robotics tasks in MuJoCo and on Atari games. With competitive performance and good  parallelization, ES algorithms are receiving more and more attention as a scalable alternative to popular MDP-based RL techniques. ES achieves fairly good performance
on challenging reinforcement learning problems and is easier to scale in a distributed setting. The objective function F measures the expected total reward of policy parameter theta.when the environment is stochastic and implemented in black-box physics simulators, the objective function F is only accessible via noisy and expensive function evaluations, and may not be smooth. So the gradient of F cannot be computed with a backpropagation-like algorithm \cite{Liu2019TrustRE}.\\
(ES) have raised attention in solving challenging tasks of modern reinforcement learning (RL) with low computation cost and high scalability. ES methods optimize the RL objective by regarding the environment as a ”blackbox”, and use the perturbed policies to explore the environment. \cite{Shi2020maxEntropy}.\\
It has been shown in those works that ES is easy to parallelize, and requires low communication overhead in a distributed setting. More importantly, being able to achieve competitive performance on many RL tasks, these methods are advantageous over other RL approaches in their high scalability and substantially lower wall-clock time. Given wide availability of distributed computing resources, all environment simulations at each iteration of training can be conducted totally in parallel. Thus, a more reasonable metric for the performance of a training algorithm is the number of non-parallelizable iterations, as opposed to the sample complexity. In this metric, ES is truly an appealing choice \cite{zhang2020accelerating}. \\
In contrast, ES techniques based on the natural gradient [5, 44, 48] are parameterization invariant and can demonstrate improved sample efficiency. 
In RL tasks, the advantages of ES – high parallelizability, better robustness, and richer exploration \cite{veer2020cones}.\\
However, ES has also several disadvantages such as: standard ES algorithms perform one gradient update per data sample, which is not very efficient. sample efficiency is lacking, which is not that high in current ES algorithm since the sampled data is only used for one gradient update \cite{Liu2019TrustRE}.\\
It is well-known that evolution strategies reinforcement learning (RL) methods suffer from low stability. Without careful consideration, ES methods are sensitive to local optima and are unstable in learning. Therefore, there is an urgent need for improving the stability of ES methods in solving RL problems. However, one major drawback for ES methods is the instability and high variance in learning. The ES gradient estimator may introduce high variance and without careful consideration, ES methods are brittle to local optima and are fragile in learning. The conventional ES for RL optimizes a deterministic policy during learning, which is not able to apply maximum entropy RL framework \cite{Shi2020maxEntropy}.\\
There are two limitations in the current ES practice that may hinder its otherwise further capabilities. First, most current methods rely on Monte Carlo type gradient estimators to suggest search direction, where the policy parameter is, in general, randomly sampled. Due to the low accuracy of such estimators, the RL training may suffer from slow convergence and require more iterations to reach optimal solution. Secondly, the landscape of reward functions can be deceptive and contains many local maxima, causing ES algorithms to prematurely converge and be unable to explore other parts of the parameter space with potentially greater rewards.
Nevertheless, there are several challenges that need to be addressed in order to further improve the performance of ES in training complex policies. First, most ES methods cope with the non-smoothness of the objective function by considering a Gaussian-smoothed version of the expected total reward. The gradient of this function is intractable
and must be estimated to provide the policy parameter update. Another prominent challenge is that the landscape of the objective function is complex and possesses plentiful local maxima. There is a risk for any optimization algorithm to get trapped in some of those points and unable to explore the parameter space effectively. One drawback of the ES method and its variants is the slow convergence of the training process, due to the low accuracy of the MC-based gradient estimator (see (Berahas et al., 2019)), also (Zhang et al., 2020), for extended discussions on the accuracy of gradient approximations using Eq. (6) and related mehods) \cite{zhang2020accelerating}. \\
Standard ES methods with d-dimensional Gaussian smoothing suffer from the curse of dimensionality due to the high variance of Monte Carlo (MC) based gradient estimators. To control the variance, Gaussian smoothing is usually limited in a small region, so existing ES methods lack nonlocal exploration ability required for escaping from local minima \cite{zhang2020novel}.\\
Standard ES methods are not invariant to re-parameterizations of the belief distribution. However, these methods have not been thoroughly exploited in RL due to the difficulties in computing the natural gradient for high-dimensional problems; in particular, the challenging estimation of the Fisher information matrix is necessary for computing the natural gradient  \cite{veer2020cones}.\\
Standard ES methods have been proved to suffer from the curse of dimensionality, due to the  random directional search and low accuracy of Monte Carlo estimation. 

\subsection{Metrics for assessing the performance of a Reinforcement Learning algorithm}
Throughout the literature, we were able to identify critical aspects for both Reinforcement learning and Evolution Strategies algorithms which are mainly considered when assessing the performance of the showcased algorithm.\\
The main aspects identified are as per the below:
\begin{itemize}
  \item Scaling
  \item Ability for adaptation, exploration
  \item Entropy, as relating to the predictability of the actions of an agent
  \item Speed of convergence
  \item Variance and data sampling
  \item Performance in Continuous control tasks
  \item Learning in a multi agent setting
\end{itemize}

\subsection{Comparing both methods via the identified metrics}
\subsubsection{Scaling and parallelism}
\paragraph{Parallelism in Evolution Strategies}
ES is well suited to be scaled up to many parallel workers: 1) It operates on complete episodes, thereby requiring only infrequent communication between workers. 2) The only information obtained by each worker is the scalar return of an episode: if we synchronize random seeds between workers before optimization, each worker knows what perturbations the other workers used, so each worker only needs to communicate a single scalar to and from each other worker to agree on a parameter update. ES thus requires extremely low bandwidth, in sharp contrast to policy gradient methods, which require workers to communicate entire gradients. 3) It does not require value function approximations. RL with value function estimation is inherently sequential: To improve upon a given policy, multiple updates to the value function are typically needed to get enough signal. Each time the policy is significantly changed, multiple iterations are necessary for the value function estimate to catch up \cite{salimans2017evolution}.\\
Highly parallelizable. ES only requires workers to communicate a few scalars between each other, while in RL it is necessary to synchronize entire parameter vectors (which can be millions of numbers). Intuitively, this is because we control the random seeds on each worker, so each worker can locally reconstruct the perturbations of the other workers. Thus, all that we need to communicate between workers is the reward of each perturbation. As a result, we observed linear speedups in our experiments as we added on the order of thousands of CPU cores to the optimization\cite{salimans2017evolution}.\\
\noindent The steps as showcased in Figure \ref{fig_parallel}are as per the below:\\
\textbf{Initialize}\\
\begin{enumerate}
  \item Create shared list of all random seeds, one per worker; and $\theta_t$
\end{enumerate}
\textbf{Repeat}\\
\begin{enumerate}
  \item Sample $\varepsilon \approx N(0,1|s_i)$
  \item Evaluate $F(\theta_t,\sigma\varepsilon_i)$
  \item Communicate F to all nodes
  \item Reconstruct $\varepsilon_i$ for all other nodes using known random seeds 
  \item $\theta_{t+1}\leftarrow \theta_t+\alpha\frac{1}{n\sigma}\sum_{j=1}^{n}F_j\varepsilon_j$
\end{enumerate}

\begin{figure*}[htbp]
\centerline{\includegraphics[width=8in]{images/parallel.png}}
\caption{Parallelization representation for Evolution Strategies \cite{salimans2017evolution}}
\label{fig_parallel}
\end{figure*}

The OpenAI Evolutionary Strategy \cite{salimans2017evolution} (OpenAI-ES) introduced several contributions for improving the training and performance and be able to compete with state-of-the-art RL algorithms, all the while renewing interest in ES methods. Additionally, the simplicity of ES made it suitable for parallel scaling across many workers and makes it scalable and efficient to use on distributed hardware \cite{salimans2017evolution}. Moreover, RL methods such as A3C need to communicate gradients back and forth between workers and a parameter server, while OpenAI-ES only requires fitness scores and high-level parameter distribution information to be communicated. \\

%Parallelism in Reinforcement Learning has been investigated widely in distributed RL \cite{nair2015massively,mnih2016asynchronous,horgan2018distributed,barthmaron2018distributed,espeholt2018impala,Zhang2019scalable,Liu2018parallel,Igor2018}.\\
%Scaling to large systems, especially dealing with many heterogeneous agents, has been a primary challenge in the RL research domain since its first days. As the world dynamics become more and more complex, this challenge has always been required to resolve. Since agents have common behaviors, such as actions, domain knowledge, and goals (homogeneous agents), the scalability can be achievable by (partially) centralized training and decentralized execution.In the heterogeneous setting with many agents, the key challenge is how to provide the most optimal solution and maximize the task completion success based on self-learning with effective coordinative and cooperative strategies among the agents. A research direction to address this difficulty is well worth an investigation. \cite{Nguyen2020_challenges}.\\

\paragraph{Parallelism in Reinforcement Learning}
\noindent Distributed RL is an efficient way that takes advantage of parallelism to achieve fast training for large complex tasks \cite{nair2015massively}. Most of the works in distributed Reinforcement Learning assume a common structure composed of multiple actors interacting with multiple copies of the same environment and a central system which stores and optimizes the common Q-function parameter or the policy parameter shared by all actors. The focus of distributed RL is to optimize the Q-function  parameter or the policy parameter fast by generating more samples for the same wall clock time with multiple actors. In order to achieve this goal, researchers investigated various techniques for distributed RL, which will be showcased below. 
        
%e.g., asynchronous update of parameters (Mnih et al. (2016), Babaeizadeh et al. (2017)), sharing an experience replay buffer (Horgan et al. (2018)), GPU-based parallel computation (Babaeizadeh et al. (2017), Clemente et al. (2017)), GPU-based simulation (Liang et al. (2018)) and V-trace in case of on-policy algorithms (Espeholt et al. (2018)).

\subparagraph{Scaling up deep reinforcement learning based on distributed asynchronous SGD: Asynchronous update of parameters }\\
In \cite{nair2015massively}, Nair et al. presented the first massively distributed architecture for deep reinforcement learning: General Reinforcement Learning Architecture (Gorila). This architecture uses four main components: parallel actors that generate new behaviour; parallel learners that are trained from stored experience; a distributed neural network to represent the value function or behaviour policy; and a distributed store of experience. 
A unique property of RL is that an agent influences the training data distribution by interacting with its environment. In order to generate more data, we deploy multiple agents running in parallel that interact with multiple instances of the same environment. Each such actor can store its own record of past experience, effectively providing a distributed experience replay memory with vastly increased capacity compared to a single machine implementation.
Alternatively this experience can be explicitly aggregated into a distributed database. In addition to generating more data, distributed actors can explore the state space more effectively, as each actor behaves according to a slightly different policy. A conceptually distinct set of distributed learners reads  samples of stored experience from the experience replay memory, and updates the value function or policy according to a given RL algorithm.
In Gorila, each process contains an actor that acts in its own copy of the environment, a separate replay memory, and a learner that samples data from the replay memory and computes gradients of the DQN loss with respect to the policy parameters. The gradients are asynchronously sent to a central parameter server which updates a central copy of the model. The updated policy parameters are sent to the actor-learners at fixed intervals. 
By using 100 separate actor-learner processes and 30 parameter server instances, a total of 130 machines, Gorila was able to significantly outperform DQN over 49 Atari games. On many games Gorila reached the score achieved by DQN over 20 times faster than DQN, and also reduced the wall-time required to achieve these results by an order of magnitude on most games. \\
In \cite{mnih2016asynchronous}, Mnih et al. provide a very different paradigm for deep reinforcement learning. Instead of experience replay, they asynchronously execute multiple agents in parallel, on multiple instances of the environment. This parallelism also decorrelates the agents’ data into a more stationary process, since at any given time-step the parallel agents will be experiencing a variety of different states. This simple idea enables a much larger spectrum of fundamental on-policy RL algorithms, such as Sarsa, n-step methods, and actorcritic methods, as well as off-policy RL algorithms such as Q-learning, to be applied robustly and effectively using deep neural networks. This  parallel reinforcement learning paradigm also offers practical benefits. Whereas previous approaches to deep reinforcement learning rely heavily on specialized hardware such as GPUs , or massively distributed architectures  \cite{nair2015massively}, the experiments in this case run on a single machine with a standard multi-core CPU. When applied to a variety of Atari 2600 domains, on many games asynchronous reinforcement learning achieves better results, in far less time than previous GPU-based algorithms, using far less resource than massively distributed approaches.\\

\subparagraph{Scaling up deep reinforcement learning: V-trace in case of on-policy algorithms}\\
One of the main challenges in training a single agent on many tasks at once is scalability. Since the current state-of the- art methods like A3C (Mnih et al., 2016) or UNREAL ) can require as much as a billion frames and multiple days to master a single domain, training them on tens of domains at once is too slow to be practical. In \cite{espeholt2018impala}, the authors developed a new distributed agent IMPALA (Importance Weighted Actor-Learner Architecture) that not only uses resources more efficiently in single machine training but also scales to thousands of machines without sacrificing data efficiency or resource utilisation. Espeholt et al. propose the Importance Weighted Actor-Learner Architecture (IMPALA) capable of scaling to thousands of machines without sacrificing training stability or data efficiency. Unlike the popular A3C-based agents, in which workers communicate gradients with respect to the parameters of the policy to a central parameter server, IMPALA actors communicate trajectories of experience (sequences of states, actions, and rewards) to a centralised learner. Since the learner in IMPALA has access to full trajectories of experience, a GPU is used to perform updates on mini-batches of trajectories while aggressively parallelising all time independent operations. This type of decoupled architecture can achieve very high throughput. However, because the policy used to generate a  trajectory can lag behind the policy on the learner by several updates at the time of gradient calculation, learning becomes off-policy. Therefore, the V-trace off-policy actor-critic algorithm is introduced to correct for this harmful discrepancy. \\
The authors demonstrate the effectiveness of IMPALA for multi-task reinforcement learning on DMLab-30 (a set of 30 tasks from the DeepMind Lab environment ) and Atari-57 (all available Atari games in Arcade Learning Environment). The results show that IMPALA is able to achieve better performance than previous agents with less data, and crucially exhibits positive transfer between tasks as a result of its multi-task approach. \\ There are different drawback to these methods however: Experience replay can only be employed with off-policy methods, while asynchronous agents can perform
inconsistent parameter updates due to stale gradients1
and simultaneous parameter updates from
different threads.

\subparagraph{Scaling up reinforcement learning by utilising GPUs: GPU-based parallel computation }
There have also been multiple efforts that scale up reinforcement learning by utilising GPUs \cite{clemente2017efficient}. Batched A2C \cite{clemente2017efficient} produces a batch of actions and applies them to a batch of environments. Therefore, the slowest environment in each batch determines the time it takes to perform the entire batch step. In other words, high variance in environment speed can severely limit performance. The authors in \cite{clemente2017efficient} propose a novel framework for efficient parallelization of deep reinforcement learning algorithms, enabling these algorithms to learn from multiple actors on a single machine. The framework is algorithm agnostic and can be applied to on-policy, off-policy, value based and policy gradient based algorithms. Given its inherent parallelism, the framework can be efficiently implemented on a GPU, allowing the usage of powerful models while significantly reducing training time.Algorithms based on this framework can learn from hundreds of actors in parallel, similar to Gorila, while running on a single machine like A3C and GA3C. Having multiple actors help decorrelate encountered states and attenuate feedback loops, while allowing the user to leverage the parallel architecture of modern CPUs and GPUs. Unlike A3C and Gorila, there is only one copy of the parameters, hence parameter updates are performed synchronously, thus avoiding the possible drawbacks related to asynchronous updates. This framework has many similarities to GA3C. However, the absence of queues allows for a much more simpler and computationally efficient solution, while allowing for true on-policy learning and faster convergence to optimal policies. 
The authors demonstrate the effectiveness of their framework by implementing an advantage actor-critic algorithm on a GPU, using on-policy experiences and employing synchronous updates. Batched A2C thus achieves state of the art performance in the Atari 2600 domain after only a few hours of training. Batched A2C works particularly well on Atari environments, because rendering and game logic are computationally very cheap in comparison to the expensive tensor operations performed by reinforcement learning agents. However, more visually or physically complex environments can be slower to simulate and can have high variance in the time required for each step. Environments may also have variable length (sub)episodes causing a slowdown when initializing an episode.

\subsubsection{Ability for adaptation and exploration}
Exploitation versus exploration is a critical topic in Reinforcement Learning. We’d like the RL agent to find the best solution as fast as possible. However, in the meantime, committing to solutions too quickly without enough exploration sounds pretty bad, as it could lead to local minima or total failure. Modern RL algorithms that optimize for the best returns can achieve good exploitation quite efficiently, while exploration remains more like an open topic.
\paragraph{Adaptation in Deep Reinforcement Learning}
Although deep RL algorithms have performed amazing feats in recent years, they have mostly done so despite relying on simple, undirected (aka dithering) exploration strategies, in which an agent hopes to explore new areas of its environment by taking random actions (e.g. epsilon-greedy exploration) \cite{conti2018improving}. When aiming to only optimize for the reward without some mechanism to encourage intelligent exploration, the algorithm may get stuck in local optima and the agent will fail to properly learn. The training data in RL is determined by the actions an agent takes. If the agent greedily takes actions that maximize reward, the training data for the algorithm will be limited and it may not discover alternate strategies with larger payoffs (i.e. it can get stuck in local optima). Sparse reward signals can also be a problem for algorithms that only maximize reward, because at times there may be no reward gradient to follow. \\

Let’s first go through several classic exploration algorithms that work out pretty well in the multi-armed bandit problem or simple tabular RL.
%https://lilianweng.github.io/lil-log/2020/06/07/exploration-strategies-in-deep-reinforcement-learning.html
\begin{itemize}
  \item Epsilon-greedy: The agent does random exploration occasionally with probability \(\epsilon\) and takes the optimal action most of the time with probability \(1-\epsilon\).
  \item Upper confidence bounds: The agent selects the greediest action to maximize the upper confidence bound \(\hat{Q}_t(a) + \hat{U}_t(a)\), where \(\hat{Q}_t(a)\) is the average rewards associated with action \(a\) up to time \(t\) and \(\hat{U}_t(a)\) is a function reversely proportional to how many times action \(a\) has been taken
  \item Boltzmann exploration: The agent draws actions from a boltzmann distribution (softmax) over the learned Q values, regulated by a temperature parameter \(\tau\).
  \item Thompson sampling: The agent keeps track of a belief over the probability of optimal actions and samples from this distribution.
\end{itemize}
A number of methods have been proposed to promote directed exploration in RL, including recent methods that handle high-dimensional state spaces with DNNs. A common idea is to encourage an agent to visit states it has rarely or never visited (or take novel actions in those states). This is done by augmenting the environment reward with an additional bonus signal to encourage extra exploration. This intrinsic reward is somewhat inspired by intrinsic motivation in psychology \cite{Oudeyer2013Intrinsic}. Exploration driven by curiosity might be an important way for children to grow and learn. In other words, exploratory activities should be rewarding intrinsically in the human mind to encourage such behavior. The intrinsic rewards could be correlated with curiosity, surprise, familiarity of the state, and many other factors \cite{Oudeyer2013Intrinsic}.
Methods proposed to track state (or state-action pair) visitation frequency include (1) approximating state visitation counts based on either auto-encoded latent codes of states or pseudo-counts from statespace density models , (2) learning a dynamics model that predicts future states (assuming predictions will be worse for rarely visited states/state-action pairs), and (3) methods based on compression (novel states should be harder to compress).
\subparagraph{Count-based Exploration}
%https://lilianweng.github.io/lil-log/2020/06/07/exploration-strategies-in-deep-reinforcement-learning.html
If we consider intrinsic rewards as rewarding conditions that surprise us, we need a way to measure whether a state is novel or appears often. One intuitive way is to count how many times a state has been encountered and to assign a bonus accordingly. The bonus guides the agent’s behavior to prefer rarely visited states to common states. This is known as the count-based exploration method. 
In \cite{tang2017exploration},  Tang et al proposes approximating state visitation counts based on auto-encoded latent codes of states. Tang et al. \cite{tang2017exploration} proposed to use Locality-Sensitive Hashing (LSH) to convert continuous, high-dimensional data to discrete hash codes. States are mapped to hash  codes, which allows to count their occurrences with a hash table. These counts are then used to compute a reward bonus according to the classic count-based
exploration theory \cite{tang2017exploration}.\\
In \cite{bellemare2016unifying,ostrovski2017countbased}, Bellemare, et al. proposes approximating state visitation counts based on pseudo-counts from statespace density models. Bellmare et al \cite{bellemare2016unifying} thus used a  simple CTS (Context Tree Switching) density model to approximate the frequency of state visits and a novel algorithm for deriving a pseudo-count from this density model. The CTS model is simple but limited in expressiveness, scalability, and data efficiency. In a following-up paper, Georg Ostrovski, et al. \cite{ostrovski2017countbased} improved the approach by training a PixelCNN as the density model.
\subparagraph{Prediction-based Exploration}
%https://lilianweng.github.io/lil-log/2020/06/07/exploration-strategies-in-deep-reinforcement-learning.html
The second category of intrinsic exploration bonuses are rewarded for improvement of the agent’s knowledge about the environment. The agent’s familiarity with the environment dynamics can be estimated through a prediction model.
%Forward Dynamics 
Learning a forward dynamics prediction model is a great way to approximate how much knowledge our model has obtained about the environment and the task MDPs. It captures an agent’s capability of predicting the consequence of its own behavior. In \cite{stadie2015incentivizing}, stadie et al. evaluate several more sophisticated exploration strategies, including Thompson sampling and Boltzman exploration, and propose a new exploration method based on assigning exploration bonuses from a concurrently learned model of the system dynamics. The authors therefore develop a scalable and efficient approach to exploration bonuses that can be applied to tasks with complex, high-dimensional state spaces. They describe a method that learns a state representation from observations, trains a dynamics model using this
representation concurrently with the policy, and uses the misprediction error in this model to asses the novelty of each state. Novel states are expected to disagree more strongly with the model than those states that have been visited frequently in the past, and assigning exploration bonuses based on this disagreement can produce rapid and effective exploration.The approach assigns model-based exploration bonuses from learned representations and dynamics, using only the observations and actions. It can scale to large problems where Bayesian approaches to exploration become impractical, and we show that it achieves significant improvement in learning speed on the task of learning to play Atari games from raw images.
In \cite{houthooft2017vime}, Houthooft proposes “Variational information maximizing exploration” (VIME), an exploration strategy based on maximization of information gain about the agent’s belief of environment dynamics. How much additional information has been obtained about the forward dynamics can be measured as the reduction in entropy. This paper proposes a curiosity-driven exploration strategy, making use of information gain about the agent’s internal belief of the dynamics model as a driving force. Within this framework, agents are encouraged
to take actions that result in states they deem surprising—i.e., states that cause large updates to the dynamics model distribution.  Experimental results show that VIME achieves significantly better performance than naïve exploration strategies.
In \cite{pathak2017curiositydriven}, Pathak et al. proposes the Intrinsic Curiosity Module which learns the state space encoding with a self-supervised inverse dynamics model. Predicting the next state given the agent’s own action is not easy, especially considering that some factors in the environment cannot be controlled by the agent or do not affect the agent. ICM believes that a good state feature space should exclude such factors because they cannot influence the agent’s behavior and thus the agent has no incentive for learning them.\\
\paragraph{Adaptation in Evolution Strategies}
Throughout this section, we will showcase the ability of Evolution Strategies to adapt to the environment they are leveraged in. 

\subparagraph{New exploration strategies for ES}
However, how to improve sample efficiency of ES algorithm is still a challenging problem. Recent methods proposed for this purpose could be divided into two categories:
(1) Adapting the search distribution by encouraging the exploration diversity. 
(2) Adapting the search distribution with the help of extra gradient information. 
In the first category, (Choromanski et al. 2018) propose to enforce orthogonality conditions on the Gaussian perturbations for parameter exploration, and they demonstrate theoretically and empirically that random orthogonal and Quasi Monte Carlo (QMC) finite difference directions are much more effective for parameter exploration than random Gaussian directions used in (Salimans et al. 2017). (Conti et al. 2017) hybridize ES with some existing algorithms which promote directed exploration like novelty search (NS) and quality diversity (QD), improving ES performance on sparse or deceptive deep RL tasks. In the second category, (Maheswaranathan et al. 2018) proposes Guided Evolution Strategies, the main idea of such method is to use extra surrogate gradient information (directions that may be correlated with, but not necessarily identical to, the true gradient) along with ES random perturbations. Specifically, they define a new search distribution for ES that is elongated along a guiding subspace spanned by the surrogate gradients. \cite{Liu2019TrustRE}

Conti et al. [2017] try to address the problems of local minima (which we also observed in games like Seaquest and Enduro) by augmenting ES algorithms with a novelty search (NS) and quality diversity (QD). Their proposed algorithms add an additional criterion to the optimization procedure that encourages exploring qualitatively different solutions during training, thus reducing the risk of getting stuck in a local optimum. The authors also propose to manage a meta-population of diverse solutions allocating resources to train more promising ones. In our experiments we observe that training runs with the same hyperparameters and different initializations often converge to achieve very different scores; managing a meta-population could therefore be an easy way to improve the results and reduce the variance between the runs. Overall, the success of Conti et al. [2017] in improving performance with some of these newer methods in ES research strengthens our expecation that a wide range of improvements to the state of the art are possible by integrating the multitude of techniques developed in ES research over the last decades into our canonical ES.

Algorithms that have been invented to promote directed exploration in small-scale evolved neural networks via populations of exploring agents, specifically novelty search (NS) and quality diversity (QD) algorithms, can be hybridized with ES to improve its performance on sparse or deceptive deep RL tasks, while retaining scalability. Throughout their paper \cite{conti2018improving}, Conti et al. introduced a family of fast, scalable algorithms for reinforcement learning that are capable of directed exploration to be hybridized with ES to scale them to deep neural networks and thus tackle hard, high-dimensional deep reinforcement learning problems, without sacrificing the speed/scalability benefits of ES. Novelty search (NS) \cite{ Lehman2011NS} and Quality diversity (QD) algorithms \cite{Pugh2016QD} have been shown to perform exploration with a population of agents rather than a single agent. Thus, the latter seemed to be a good fit for ES which  recently shown to perform well on high-dimensional deep RL tasks in a short amount of wall clock time by scaling well to many distributed computers \cite{salimans2017evolution}. \\
Conti et al. thus studied NS, which performs exploration only (ignoring the reward function) to find a set of novel solutions, then investigated algorithms that balance exploration and exploitation, specifically novel instances of QD algorithms, which seek to produce a set of solutions that are both novel and high-performing. 
Inspired by nature’s drive towards diversity, NS encourages policies to engage in notably different behaviors than those previously seen. The algorithm encourages different behaviors by computing the novelty of the current policy with respect to previously generated policies and then encourages the population distribution to move towards areas of parameter space with high novelty. NS outperforms reward-based methods in maze and biped walking domains, which possess deceptive reward signals that attract agents to local optima.
NS-ES alone can enable agents to avoid deceptive local optima in the reward function. Reward signals, however, are still very informative and discarding them completely may cause performance  to suffer. Consequently, Conti et al. trained a variant of NS-ES, called NSR-ES, that combines the reward (“fitness") and novelty calculated for a given set of policy parameters $\theta$. Similar to NS-ES and ES, NSR-ES operates on entire episodes and can thus evaluate reward and novelty simultaneously for any sampled parameter vector.
As with any exploration method, encouraging novelty can come at a cost if such an exploration pressure is not necessary. In Atari games such as Alien and  Gravitar, and in the Humanoid Locomotion problem without a deceptive trap, both NS-ES and NSR-ES perform worse than ES. To avoid this cost, the authors introduced the NSRA-ES algorithm, which attempts to invest in exploration only when necessary. NSRA-ES tends to produce better results than ES, NS-ES, and NSR-ES across many different domains, making it an attractive new algorithm for deep RL tasks. Similar strategies for adapting the amount of exploration online may also be advantageous for other deep RL algorithms. The experiments confirm that NS-ES and two simple versions of QD-ES (NSR-ES and NSRA-ES) avoid local optima encountered by ES and achieve higher performance and avoid local optima  on tasks ranging from simulated robots learning to walk around a deceptive trap to the high-dimensional pixel-to-action task of playing Atari games. 

In \cite{zhang2018comparing}, Zhang et al. conduct a comparison
between the state-of-the-art techniques in both Deep Reinforcement Learning and Evolutionary Methods in Continuous Control n in terms of both wall time and environment time steps, i.e. the amount of interactions with the environment, to gain
a better empirical understanding of the running speed and data efficiency of all the algorithms. After many experiments, no algorithm was proved to consistently outperform others across all tasks. However, most deep RL methods appeared to get trapped in some local minima, which denotes that evolutionary methods are
better at exploration than the deep RL methods. Moreover, in some tasks, 
where rich dynamics are involved, most deep RL methods worked better and many evolutionary methods appeared to get trapped in some local minima, which denotes that the deep RL methods can handle rich dynamics better than the evolutionary methods. 

\subparagraph{Independent Gaussian samples}
We found that ES exhibited better exploration behaviour than policy gradient methods like TRPO: on the MuJoCo humanoid task, ES has been able to learn a very wide variety of gaits (such as walking sideways or walking backwards). These unusual gaits are never observed with TRPO, which suggests a qualitatively different exploration behavior.  Whereas RL algorithms like Q-learning and policy gradients explore by sampling actions from a stochastic policy, Evolution Strategies derives learning signal from sampling instantiations of policy parameters. Exploration in ES is thus driven by parameter perturbation. For ES to improve upon parameters θ, some members of the population must achieve better return than others: i.e. it is crucial that Gaussian perturbation vectors $\varepsilon$ occasionally lead to new individuals $\theta + \sigma\varepsilon$ with better return \cite{salimans2017evolution}

\subparagraph{Quasi Monte Carlo (MC) estimators}

In \cite{choromanski2018structured},  Choromanski et al. propose "Structured Exploration". Moreover the authors show both theoretically and empirically that random orthogonal and Quasi Monte Carlo (QMC) finite difference directions are
much more effective for parameter exploration than random Gaussian directions used in \cite{salimans2017evolution}. It was therefore shown that Structured exploration can be successfully applied to provide scalable blackbox optimization algorithms and used in reinforcement learning to learn good quality policies.

In \cite{choromanski2019complexity}, present a new algorithm (ASEBO) for optimizing high-dimensional blackbox functions. ASEBO adapts to the geometry of the function and learns optimal sets of sensing directions, which are used to probe it, on-the-fly. It addresses the exploration-exploitation trade-off of blackbox optimization with expensive blackbox queries by continuously learning the bias of the lower-dimensional model used to approximate gradients of smoothings of the function via compressed sensing and contextual bandits methods.

Standard ES methods with d-dimensional Gaussian smoothing suffer from the curse of dimensionality due to the high variance of Monte Carlo (MC) based gradient estimators. To control the variance, Gaussian smoothing is usually limited in a small region, so existing ES methods lack nonlocal exploration ability required for escaping from local minima. In \cite{zhang2020novel}, the authors propose an improved evolution strategy (DGS-based ES algorithm as DGS-ES method) using a novel nonlocal gradient operator for high-dimensional black-box optimization. By developing this method based on directional Gaussian smoothing (DGS),  use it to replace the standard GS operator in ES to enhance nonlocal exploration in high dimensions. The authors develop a nonlocal gradient operator with directional Gaussian smoothing (DGS) to address this challenge.  This method enables effective nonlocal exploration to facilitate the global search in high-dimensional optimization.  Moreover, they develop an accurate estimator for the DGS gradient using Gauss-Hermite  quadrature, which accelerates the convergence of ES. 

\subsection{Variance and data sampling}

==> sections/draft/conceptualOverview.tex <==
Throughout this section, we will introduce the concepts of Reinforcement Learning, Deep Reinforcement Learning and Evolution Strategies: their basic elements, concepts and terminology, and a high level explanation of their underlying algorithms.

\subsection{Reinforcement learning}
\textbf{\textit{RL Overview.}} Reinforcement learning is a branch of Machine Learning where an algorithm (also knows as "agent") learns via trial-and-error while interacting with the environment it is in \cite{Kaelbling1996}, as seen in Figure \ref{RL_fig}.
The Reinforcement Learning (RL) process can be modeled as a cycle as shown in Figure \ref{fig:drl_problem_setup}:
\begin{itemize}
  \item The agent observes the environment
  \item The Agent sends an action to the Environment based on a specific policy in an attempt to control it in a favorable way (step 2)
  \item The environment transitions to a new state (step 3)
  \item The agent receives an observation (also knows as "state") and reward from the environment (Step 4)
  \item The Learning algorithm uses this state and reward for deciding the next action to take (Step 5)
\end{itemize}

\begin{figure}[htbp]
\centerline{\includegraphics[width=3in]{images/RL_general.png}}
\caption{Reinforcement Learning}
\label{RL_fig}
\end{figure}

Table \ref{RL_def} below summarizes the main elements of Reinforcement Learning along with their notations.

\begin{table*}[htbp]
\caption{basic elements of Reinforcement Learning}
\begin{center}
\label{RL_def}
\begin{tabular}{p{0.22\linewidth} | p{0.10\linewidth} | p{0.60\linewidth}}
 \hline 
 Element & Notation & Short description \\
 \hline\hline  
 Agent & N/A & Computer program or algorithm\\ 
 \hline
  Environment & N/A &  Everything the agents interacts with is called an environment. The environment is the outside world. It comprises everything outside the agent \cite{sutton2018reinforcement}\\
 \hline
  Action & $a$ & Decision taken by the agent \cite{sutton2018reinforcement}\\ 
 \hline
  State & $s$ & The Environment is represented by a set of variables related to the problem. This set of variables and all the possible values they can take are referred to as the state space. A state is an instantiation of the state space, a set of values the variables take \cite{sutton2018reinforcement}\\ 
 \hline
  Observation & N/A & The state of the environment as seen by the agent \cite{sutton2018reinforcement}\\
   \hline
    Policy & $\pi$ & a mapping from states to probabilities of selecting each possible action \cite{sutton2018reinforcement}\\ 
 \hline
  Reward & $r$ & Scalar value provided to the agent as a direct answer to its actions\\ 
 \hline
   Return & $G$ & It is the sum of discount future rewards. \cite{sutton2018reinforcement}\\ 
 \hline
  State-value function & $v_\pi(s)$ & It is the expected return from a given state, $s$, and following a specific policy, $\pi$, thereafter.  \cite{sutton2018reinforcement}\\ 
 \hline
%   Optimal state-value function & $v_*(s)$ & Value of state $s$ under the optimal policy\cite{Sutton1998}\\ 
%  \hline
  Action-value function & $q_\pi(s,a)$ & It is the expected return of taking a particular action, $a$, in a state, $s$, and follow a specific policy, $\pi$, thereafter~\cite{sutton2018reinforcement}\\
%  \hline
%   Optimal action-value function & $q_*(s,a)$ & Value of taking action $a$ in state $s$ under the optimal policy\cite{Sutton1998}\\
 \hline
  Dynamic programming & DP & Method for solving complex problems by breaking them down into subproblems. Consists of first solving the subproblems then combing the solutions to the latter\cite{Sutton1998}\\ 
 \hline
  Monte Carlo methods & MC & Monte Carlo methods are ways of solving the reinforcement learning problem based on averaging sample returns. Only on the completion of an episode are value estimates and policies changed \cite{Sutton1998}\\ 
 \hline
 Temporal Difference &  TD & TD learning is a combination of Monte Carlo ideas and dynamic programming (DP) ideas. Like Monte Carlo methods, TD methods can learn directly from raw experience without a model of the environment’s dynamics. Like DP, TD methods update estimates based in part on other learned estimates, without waiting for a final outcome  \cite{Sutton1998}\\ 
 \hline
 On-policy methods & N/A & Evaluate or improve the behaviour policy  that the agent is already using for action selection (i.e. SARSA)\\
 \hline
 Off-policy methods & N/A &  learn an optimal value function/policy, that could follow an unrelated behaviour policy than the one used for action selection (i.e. q-learning)\\ 
 \hline
 Epsilon-greedy policy & $\varepsilon$-greedy &  We will define that a policy is $\varepsilon$-greedy with respect to an action-value function estimate Q if for every state, with probability $1-\varepsilon$, the Agent selects the greedy action, and with probability $\varepsilon$, the Agent selects an action uniformly at random from the set of available (non-greedy and greedy) actions.\\
 \hline
 stochastic policy & N/A &  A stochastic policy outputs a probability distribution over actions.\\
 \hline
 Deterministic policy & N/A &  A deterministic policy is policy that maps state to actions. You give it a state and the function returns an action to take.\\
 \hline
\end{tabular}
\label{tab1}
\end{center}
\end{table*}

%https://www.analyticsvidhya.com/blog/2020/11/reinforce-algorithm-taking-baby-steps-in-reinforcement-learning/
\noindent A reinforcement learning problem is usually set up as a Markov Decision Process (MDP). In its simplest form, an MDP consist of an agent, a set of states, a set of actions, a state-transition model and a reward function. The agent acts in the environment by taking actions which allow him to transition between states. The state-transition model describes for every action the probability of ending up in each of the states. The reward function specifies the \textit{immediate} reward obtained after transitioning from a state to another state. \\
\noindent There are two main strategies to solve MDP problems, model-based, and model-free.  Despite their data efficiency, model-based methods (e.g., dynamic programming methods) require full knowledge of the environment to plan an optimal solution. Therefore, they face difficulty tackling complex problems with large and unknown environments. Model-free methods, on the other hand, do not require full knowledge of the environment and aim at learning a policy to maximize the agent's long term cumulative reward~\cite{ding2020introduction}. The final policy which maximizes the long-term reward is called an optimal policy. \\
\noindent There are two approaches to train our agent to find this optimal policy $\pi^*$:
\begin{itemize}
\item \textit{Value-based optimization algorithms} In Value based methods, instead of training a policy function, we train a value function that maps a state to the expected value of being at that state. The value of a state is the expected discounted return the agent can get if it starts in that state, and then act according to our policy. It teaches the agent to learn which state is more valuable and then takes the action that leads to the more valuable states. Examples of such algorithms are value iteration~\cite{valueiter}, Q-learning, DQN~\cite{DQN}, and SARSA~\cite{SARSA}.
\item \textit{Policy-based optimization algorithms} In Policy-Based Methods, we learn a policy function directly by teaching the agent to learn which action to take, given the state it is in. This function will map from each state to the best corresponding action at that state. Examples of such algorithms are policy iteration~\cite{policyiter}, policy gradient~\cite{policygradient} and REINFORCE~\cite{reinforce}. In contrast to value-based methods like TD learning and Q-learning, policy-based methods optimize the policy $\pi(a|s;\theta)$ (with function approximation) directly, and update the parameters $\theta$ by gradient ascent \cite{li2018deep}.
\end{itemize}

\noindent Both of these approaches have their advantages. Value-based algorithms are sample efficient and steady while policy-based methods in comparison usually have better convergence properties, and are effective in high-dimensional or continuous action spaces, and can learn stochastic policies\cite{li2018deep}. \\

\textbf{\textit{Common RL algorithms.}} This section will go over the main Reinforcement Learning algorithms, covering them at a high level.\\

% The aim behind SARSA is to estimate $Q_\pi(s, a)$ for the current policy $\pi$ and all state-action (s-a) pairs. This is done by using the TD update rule applied at every timestep by letting the agent transition from one state-action pair to another state-action pair. SARSA evaluates the policy based on samples from the same policy, then refines the policy greedily with respect to action values \cite{li2018deep}.

%https://www.cse.unsw.edu.au/~cs9417ml/RL1/algorithms.html
% This procedural approach of SARSA can be translated into plain english steps as follows:
% \begin{algorithm}
% \SetAlgoLined
% Initialize $Q(s, a)$ arbitrarily\\
% \For{each episode}{
%     Observe the current state  $s$\\
%     \For{each step of episode until $S$ is terminal}{
%       Choose an action, $a$, for that state based on one of the action selection policies ($\varepsilon$-soft, $\varepsilon$-greedy or softmax).\\
%       Take the action, and observe the reward, $r$, as well as the new state, $s'$.\\
%       \textbf {A new action, and therefore reward, is selected using the same policy that determined the original action. Updating the Q-value is done according to the formula and parameters described above in equation (\ref{eq_sarsa})}\\
%       Set the state to the new state, and repeat the process until a terminal state is reached.\\
%     }
% }
%  \caption{SARSA for estimating $Q\approx q_*$ \cite{Sutton1998}}
% \end{algorithm}
%\noindent The value of $\varepsilon$ determines the exploration-exploitation of the agent.
%If $\varepsilon$ is large, the random number $r$ will hardly ever be larger than $\varepsilon$ and a random action will hardly ever be taken (less exploration, more exploitation)
%If $\varepsilon$ is small, the random number $r$ will often be larger than $\varepsilon$ which will cause the agent to choose more random actions. This stochastic characteristic will allow the agent to explore the environment even more.
%As a rule of thumb, $\varepsilon$ is usually chosen to be 0.9 but can be varied depending upon the type of environment. In some cases, $\varepsilon$ is annealed over time to allow higher exploration followed by higher exploitation.\\
%\begin{algorithm*}
%\SetAlgoLined
% Algorithm parameters: step size $\alpha \in (0,1], small  \varepsilon > 0$
% Initialize $Q(s, a)$, for all $s \in S^+$, $a \in A(s)$, arbitrarily except that %$Q(terminal, ·) = 0$\;
% \For{each episode}{
%  Initialize S\;
%  Choose A from S using policy derived from Q (e.g., $ \varepsilon-greedy$)\;
%  \For{each step of episode until S is terminal}{
%   Take action $A$, observe $R$, $S'$\;
%   Choose $A'$ from $S'$ using policy derived from $Q$ (e.g., $\varepsilon-greedy$)\;
%   $Q(S,A)\leftarrow Q(S,A)+\alpha(R+\gamma Q(S',A')-Q(S,A))$\;
%   $S \leftarrow S'$ ; $A \leftarrow A'$ \;
%   }{
%  }
% }
% \caption{SARSA for estimating $Q\approx q_*$ \cite{Sutton1998}}
%\end{algorithm*}

The Q-Learning \cite{watkins_1989} algorithm is an off-policy (uses a different policy for acting and updating), model-free RL algorithm. It is a primitive form of Reinforcement Learning which leverages Q-values to iteratively optimize the behavior of the learning agent.\\
This procedural approach of Q-Learning can be translated into the following Figure \ref{q_learning} which steps are explained below: \\
\begin{figure}[htbp]
\centerline{\includegraphics[width=3in]{images/q_learning.png}}
\caption{Q-Learning algorithm}
\label{q_learning}
\end{figure}
The general idea behind q-learning is as follows :
\begin{itemize} 
  \item The Q-Learning algorithm trains the Q-Function, an action-value function that contains, as internal memory, a Q-table that contains all the state-action pair values.
  \item Given a state and action, our Q-Function will search into its Q-table the corresponding value.
  \item When the training is done, we have an optimal Q-Function, so an optimal Q-Table.
  \item And if we have an optimal Q-function, we have an optimal policy, since we know for each state, what is the best action to take.
\end{itemize}

\noindent The Q-Learning algorithm is explained in plain English below:
\begin{enumerate}
    \item Initialize the Q-Table for each state-action pair. Most of the time we initialize the values to 0.
    \item Choose an action $A_t$ using the Epsilon Greedy Strategy (handles the exploration/exploitation trade-off): At the beginning of the training, the probability of doing exploration will be very big since $\varepsilon$ is very high, so most of the time we’ll explore. But as the training goes on, and consequently our Q-Table gets better and better in its estimations, we progressively reduce the epsilon value since we will need less and less exploration and more exploitation.
    \item Perform action $A_t$, gets $R_{t+1}$ and $S_{t+1}$
    \item in TD Learning, we update our policy or value function after one step of interaction. To produce our TD target, we used the immediate reward $R_{t+1}$ plus the discounted value of the next state best state-action pair. We thus update $Q(S_t, A_t)$ using the Q-Learning update rule:
    \begin{multline}
    Q(s_t,a_t)\leftarrow Q(s_t,a_t)+\alpha(r_{(t+1)}+\\
    \gamma max_a Q(s_{(t+1)},a_{(t+1)})-Q(s_t,a_t))
    \label{eq_qlearning}
    \end{multline}
    In this formula, $\alpha$ is the learning rate, $r_{(t+1)}$ is the immediate reward, and $\gamma max_a Q(s_{(t+1)},a_{(t+1)})$ is the discounted estimate optimal Q-value of the next state. The best next-state-action pair value, is selected with a greedy-policy (the action that has the highest state-action value) rather than the epsilon greedy policy.
\end{enumerate}


The State-Action-Reward-State'-Action' (SARSA) algorithm leverages TD for evaluation or prediction.It is an on-policy (uses the same policy for acting and updating), model-free RL algorithm.  It’s  exactly  like  Q-Learning  except that it’s the Epsilon-Greedy Policy that selects the next state-action pair, not a greedy-policy. Figure \ref{SARSA} represents the trajectory when using SARSA.
%https://towardsdatascience.com/mc-control-methods-50c018271553
\noindent The Temporal Difference formula for SARSA thus becomes :\\ 
\begin{multline}
Q(s_t,a_t)\leftarrow Q(s_t,a_t)+\alpha(r_{(t+1)}\\+\gamma Q(s_{(t+1)},a_{(t+1)})-Q(s_t,a_t))
\label{eq_sarsa}
\end{multline}

\begin{figure}[htbp]
\centerline{\includegraphics[width=3.7in]{images/SARSA.png}}
\caption{SARSA explained}
\label{SARSA}
\end{figure}

%\begin{algorithm*}
%\SetAlgoLined
% Algorithm parameters: step size $\alpha \in (0,1], small  \varepsilon > 0$
% Initialize $Q(s, a)$, for all $s \in S^+$, $a \in A(s)$, arbitrarily except that %$Q(terminal, ·) = 0$\;
% \For{each episode}{
%  Initialize S\;
%  \For{each step of episode until S is terminal}{
%   Choose A from S using policy derived from Q (e.g., $ \varepsilon-greedy$)\;
%   Take action $A$, observe $R$, $S'$\;
%   Choose $A'$ from $S'$ using policy derived from $Q$ (e.g., $\varepsilon-greedy$)\;
%   $Q(S,A)\leftarrow Q(S,A)+\alpha(R+\gamma max_a Q(S',a)-Q(S,A))$ \;
%   $S \leftarrow S'$\;
%   }{
%  }
% }
% \caption{Q-Learning for estimating $\pi \approx \pi_*$ \cite{Sutton1998}}
%\end{algorithm*}\\

%https://www.cse.unsw.edu.au/~cs9417ml/RL1/algorithms.html


% \begin{algorithm}
% \SetAlgoLined
% Initialize $Q(s, a)$ arbitrarily\\
% \For{each episode}{
%     Observe the current state  s\\
%     \For{each step of episode until S is terminal}{
%       Choose an action, a, for that state based on one of the action selection policies (-soft, -greedy or softmax).\\
%       Take the action, and observe the reward, r, as well as the new state, s'.\\
%       \textbf{Update the Q-value for the state using the observed reward and the maximum reward possible for the next state. The updating is done according to the formula and parameters described above in equation (\ref{eq_qlearning}).}\\
%       Set the state to the new state, and repeat the process until a terminal state is reached.\\
%     }
% }
%  \caption{Q-Learning for estimating $\pi \approx \pi_*$ \cite{Sutton1998}}
% \end{algorithm}

%https://towardsdatascience.com/policy-based-methods-8ae60927a78d

With value-based methods, the Agent uses its experience with the Environment to maintain an estimate of the optimal action-value function. The optimal policy is then obtained from the optimal action-value function estimate (e.g., using $\varepsilon$-greedy).\\
Instead, Policy-based methods directly learns the optimal policy from the interactions with the environment, without having to maintain a separate value function estimate.\\

% Policy gradient is thus another approach to solving reinforcement learning problems. The policy gradient methods target at modeling and optimizing the policy directly. The policy is usually modeled with a parameterized function with respect to $\theta$. $\pi_\theta(a|s)$ is therefore the probability of taking action $a$ in state $s$. $\theta$ represents the parameters of the policy (the weights of the neural network).Since $\theta$ will change, the notation $\theta_t$ is used to denote $\theta$ at iteration $t$.
% The final goal thus becomes to update $\theta$ to values that make $\pi_\theta(a|s)$ the optimal policy (using the update rule from $\theta_t$ to $\theta_t+1$)\\
% Typically, for a discrete action space, $\pi_\theta$ would be a neural network with a softmax output unit, so that the output can be thought of as the probability of taking each action. Clearly, if action $a\ast$ is the optimal action, $\pi_\theta(a\ast|s)$ will have to be as close to 1 as possible.\\
% For this a simple gradient ascent can be performed on $\pi_\theta(a*|s)$, so that at each iteration $\theta$ is updated in the following way:\\
% \begin{equation}
% \theta_{t+1}=\theta_t+\alpha\delta\pi_\theta_t(a\ast|s)
% \label{eq_policyGrad}
% \end{equation}
% The gradient $\delta\pi_\theta_t(a\ast|s)$ can be seen as being “the direction in which to move $\theta_t$ so as to increase the value of $\pi_\theta t(a|s)$ the fastest”. This would help "push" more towards $a\ast$ in our policy. Since we don't know the optimal action, we thus need to push  on actions in a way that is proportional to our guess of the value of these actions. This guess of the value of action $a$ in state $s$ is $\hat{Q} (s,a$) and we get:\\
% \begin{equation}
% \theta_{t+1}=\theta_t+\alpha \hat{Q}(s,a) \delta\pi_\theta_t(a\ast|s)
% \label{eq_policyGrad}
% \end{equation}
% However, since the policy used has a hand in the choice of actions, a "policy correction" needs to be made giving the update rule below:\\
% \begin{equation}
% \theta_{t+1}=\theta_t+\alpha \frac{(\hat{Q}(s,a) \delta\pi_\theta_t(a\ast|s))}{\pi_\theta_t(a^\ast|s)}
% \label{eq_policyGrad}
% \end{equation}
The key idea underlying policy gradients is reinforcing good actions: to push up the probabilities of actions that lead to higher return, and push down the probabilities of actions that lead to a lower return, until you arrive at the optimal policy. \\
We will thus go through the REINFORCE algorithm \cite{WilliamsREINFORCE1992}. REINFORCE is one of the fundamental policy gradient algorithms on which nearly all the advanced policy gradient algorithms are based.\\
The concepts below are critical for understanding REINFORCE:
\begin{itemize}
  \item  \textit{The trajectory ($\tau$).} $\tau$ is a state-action-reward sequence (reward is ignored). It is a bit more flexible than the episode as there are no restrictions on its length (it can correspond to a full episode or just a part of an episode- we denote the length with a capital H, where H stands for Horizon) i.e. $\tau$: $\tau=(s_0,a_0,r_1,s_1,a_1,r_2,...,a_H,r_{H+1},s_{H+1})$
  \item  \textit{The return for a trajectory $R(\tau)$.} $R(\tau)$ is calculated as the sum reward from that trajectory $\tau$. i.e. $R(\tau)=(G_0,G_1,...G_H)$. The parameter $G_k$ is called the total return, or future return, at time step $k$ for the transition $k$ i.e. $(s_k,a_k,r_{k+1})$
  \item \textit{The expected return $U(\theta)$.} The goal of this algorithm is to find the weights $\theta$ of the neural network that maximize the expected return $U(\theta)$. One way to determine the value of $\theta$ that maximizes the $U(\theta)$ function is through gradient ascent. The update step for gradient ascent can be expressed as:  $\theta \leftarrow \theta + \alpha \delta_\theta U(\theta)$
  %i.e. $U(\theta)=\sum_{tau}P(\tau;\theta)R(\tau)$. 
\end{itemize}
The agent collects a trajectory $\tau$ using its current policy, and uses it to update the policy parameter. The REINFORCE algorithm is based on trial and error: a rollout $\tau$ is sampled. If it generates a high reward, its likeliness is increased, else it is decreased. This can be seen as stochastic gradient ascent on $R(\tau)$.\\
\noindent The steps involved in the implementation of REINFORCE would be as follows:
\begin{enumerate}
    \item Initialize a Random Policy (a NN that takes the state as input and returns the probability of the actions)
    \item Use the policy to collect a trajectory $\tau=(s_0,a_0,r_1,s_1,a_1,r_2,...,a_H,r_{H+1},s_{H+1})$
    \item Estimate the return for this trajectory - $R(\tau)=(G_0,G_1,...G_H)$
    \item Use the trajectory to estimate the gradient $\delta_\theta U(\theta)$
    \item Adjust weights $\theta$ of Policy (back-propagate error in Neural Network)
    \item Repeat from 2
\end{enumerate}


% This procedural approach of REINFORCE can be translated into plain english steps as follows:
% \begin{algorithm}
% \SetAlgoLined
% Input a differentiable policy parameterization $\pi(a \mid s, \theta)$\\
% Define step-size $\alpha > 0$\\
% Initialize policy parameters $\theta \in \rm I\!R^d$\\
% \For{each episode (or forever)}{
%     Generate an episode $s_0, a_0, r_1…,s_{T-1},a_{T-1}, r_T$, following $\pi(a \mid s, \theta)$\\
%     \For{$t=1$ to $T-1$ do}{
%       $G_t \leftarrow$ return from step $t$ \\
%       \\Updating the weights $\theta$ of the policy \\
%       $\theta \leftarrow \theta + \alpha \delta_\theta log \pi_\theta (s_t,a_t)v_t$\\
%     }
% }
%  \caption{REINFORCE algorithm \cite{WilliamsREINFORCE1992}}
% \end{algorithm}



\begin{figure}[htbp]
\centerline{\includegraphics[width=3.7in]{images/REINFORCE.png}}
\caption{REINFORCE explained}
\label{REINFORCE}
\end{figure}

\subsection{Deep Reinforcement learning}

\textbf{\textit{DRL Overview.}} Deep Reinforcement learning, which was first introduced in 2015 by \citet{Mnih2015} has proven to be adequate for handling highly dimensional input data. It is the combination of Reinforcement Learning and Deep Learning, and is being used to solve a wide range of complex decision-making tasks that were previously out of reach for a machine to solve real-world problems with human-like intelligence. Deep RL combines the ability to process highly-dimensional  input using a deep neural network with the flexibility of reinforcement learning to produce a highly scalable and adaptive system. After training, the resulting model can be copied and distributed over any number of agents.\\ 
\begin{figure}[htbp]
\centerline{\includegraphics[width=\columnwidth]{images/DRL.png}}
\caption{Deep Reinforcement learning}
\label{DRL_fig}
\end{figure}
We obtain deep reinforcement learning (deep RL) methods when we use deep neural networks to represent the state or observation, and/or to approximate any of the following components of reinforcement learning: value function, $v(s; \theta)$ or $q(s, a; \theta)$, policy $π(a|s; \theta)$, and model (state transition function and reward function) as seen in Figure \ref{DRL_fig}. Here, the parameters $\theta$ are the weights in deep neural networks.We usually utilize stochastic gradient descent to update weight parameters in deep RL. Recent work like deep Q-network \cite{Mnih2015} and AlphaGo \cite{Silver2016Go} stabilize the learning and achieve outstanding results. \\
As previously mentioned,stochastic gradient descent is mainly used for relatively efficient learning. It is still however extremely sensitive to hyperparameter choices and does not have good convergence properties \cite{Bruin2020IFAC}. Gradient-free optimization are therefore also proposed as of late such as Evolution Strategies which we will be looking at in the next section. The latter can adequately cater for low-dimensional parameter spaces but faces some difficulties when applied to large networks with a large number of parameters.

\textbf{\textit{Common algorithms.}} In the following, we first introduce Deep Q-Network (DQN) (Mnih et al., 2015), a recent breakthrough, and its extensions. DQN ignited this wave of deep reinforcement learning, combating the stability and convergence issues with experience replay and target networks, which make Q-learning closer to supervised learning.\\
DQN makes several contributions: 
\begin{enumerate}
    \item Stabilizing the training of action value function approximation with deep neural networks, in particular, CNNs, using experience replay and target network
    \item Designing an end to-end RL approach (i.e. only the pixels and the game score are inputs in the Atari testbed, so that only minimal domain knowledge is required)
    \item Training a flexible network with the same algorithm, network architecture and hyperparameters to perform well on many different tasks
\end{enumerate}
% 1) stabilizing the training of action value function approximation with deep neural networks, in particular, CNNs, using experience replay and target network; 2) designing an end to-end RL approach, with only the pixels and the game score as inputs, so that only minimal domain knowledge is required; 3) training a flexible network with the same algorithm, network architecture and hyperparameters to perform well on many different tasks, i.e., 49 Atari games , outperforming previous algorithms, and performing comparably to a human professional tester. \\
Experience Replay stores experiences including state transitions, rewards and actions (i.e. $e_t=(s_t,a_t,r_t,s_{t+1})$ ), which are necessary data to perform Q learning, and makes mini-batches to update neural networks.\\
In DQN, we replace the Q Learning’s table with a neural network that tries to approximate Q Values. It is usually referred to as the approximator or the approximating function, and denoted as $Q(s,a; \theta)$, where $\theta$ represents the trainable weights of the network. As seen in Figure \ref{DQN_fig}, $Q(s,a; \theta_k)$ is initialized to random values (close to 0) everywhere in its domain and the replay memory is initially empty; the target Q-network parameters $\theta_k^-$ are only updated every C iterations with the Q-network parameters $\theta_k$ and are held fixed between updates; the update uses a mini-batch (e.g., 32 elements) of tuples $< s, a >$ taken randomly in the replay memory along with the corresponding mini-batch of target values for the tuples.
% \begin{figure}[htbp]
% \centerline{\includegraphics[width=\columnwidth]{images/DQN.png}}
% \caption{Deep Q-networks}
% \label{DQN_fig}
% \end{figure}

\begin{figure}[htbp]
\centerline{\includegraphics[width=\columnwidth]{images/DQN_img.png}}
\caption{Deep Q-networks}
\label{DQN_fig}
\end{figure}

% https://medium.com/@markus.x.buchholz/deep-reinforcement-learning-deep-deterministic-policy-gradient-ddpg-algoritm-5a823da91b43
% \noindent Another algorithm is the Deep Deterministic Policy Gradient (DDPG) \cite{Khadka2018,lillicrap2019continuous}. Policy gradient methods frame the goal of maximizing return as the minimization of a loss function $L(\theta)$ where $\theta$ parameterizes the agent. A widely used policy gradient method is Deep Deterministic Policy Gradient (DDPG) [33], a model-free RL algorithm developed for working with continuous high dimensional actions spaces. DDPG uses an actor-critic architecture \cite{Sutton1998deep} maintaining a deterministic policy (actor) $\pi;S\rightarrow A$, and an action-value function approximation (critic) $Q : S × A \rightarrow R$.
% The critic’s job is to approximate the actor’s action-value function $Q^\pi$ . Both the actor and the critic are parameterized by (deep) neural networks with $\theta^\pi$
% and $\theta^Q$, respectively. A separate copy of the actor $\pi'$ and critic $Q'$ networks are kept as target networks for stability. These networks are updated
% periodically using the actor $\pi$ and critic networks $Q$ modulated by a weighting parameter $\tau$ .\\
% A behavioral policy is used to explore during training. The behavioral policy is simply a noisy version of the policy: $\pi_b(s)=\pi(s)+N(0,1)$, where $N$ is temporally correlated noise generated using the Ornstein-Uhlenbeck process \cite{Uhlenbeck}. The behavior policy is used to generate experience in the
% environment. After each action, the tuple $(s_t, a_t, r_t, s_{t+1})$ containing the current state, actor’s action, observed reward and the next state, respectively is saved into a cyclic replay buffer $R$. The actor and critic networks are updated by randomly sampling mini-batches from $R$. The critic is trained by minimizing the loss function:\\
% $L=\frac{1}{T}\sum_i(y_i-Q(s_i,a_i|\theta^Q))^2 $\\ where $ y_i=r_i+\gamma Q'(s_{i+1},\pi'(s_{i+1}|\theta^\pi')|\theta^{Q'})$\\
%The actor is trained using the sampled policy gradient:\\
% \begin{algorithm*}
% \SetAlgoLined
% \SetKwInOut{Input}{Input}\SetKwInOut{Output}{Output}
% \Input{the pixels and the game score}
% \Output{Q action value function (from which we obtain a policy and select actions)}
%  initialize replay memory $D$\\
%  initialize action-value function $Q$ with random weight $\theta$\\
%  initialize target action-value function $\hat{\theta}$ with weights $\theta^-=\theta$\\
%  \For{episode = 1 to M}{
%   initialize sequence $s1 = {x_1}$ and preprocessed sequence $\phi_1 = \phi(s_1)$\\
%   \For{t = 1 to T}{
  
% \mathleft
%     \begin{equation}
%       \text{following $\varepsilon$-greedy policy, select } &  a_t=
%         \begin{cases}
%           \text{a random action with probability $\varepsilon$}\\
%           \text{argmax_a $Q(\phi(s_t),a;\theta)$}\\
%         \end{cases}       
%     \end{equation}
%     execute action $a_i$ in emulator and observe reward $r_t$ and image $x_{t+1}$\\
%     set $s_{t+1} = s_t$, $a_t, x_{t+1}$ and preprocess $\phi_{t+1} = \phi(s_{t+1})$\\
%     store transition $(\phi_t, a_t, r_t, \phi_{t+1})$ in $D$\\
%     // experience replay \\
%     sample random minibatch of transitions $(\phi_j , a_j , r_j , \phi_j+1)$ from $D$\\
%     \begin{equation}
%       \text{set } &  y_j=
%         \begin{cases}
%           \text{$r_j$ if episode terminated at step $j+1$}\\
%           \text{$r_j+\gamma max_{a'}\hat{Q}(\phi_{j+1},a';\theta^-)$ otherwise}\\
%         \end{cases}       
%     \end{equation}
%     perform a gradient descent step on $(y_j − Q(\theta_j , a_j ; \theta))_2$ w.r.t. the network parameter $\theta$\\
%     // periodic update of target network \\
%     in every C steps, reset $\hat{Q} = Q$, i.e., set $\theta^-= \theta$\\
%   }{
%   }
%  }
%  \caption{Deep Q-Nework (DQN), adapted from Mnih et al. \cite{mnih2013playing}}
% \end{algorithm*}\\

\subsection{Evolutionary Strategies}
\textbf{\textit{ES Overview.}} Evolution Strategies (ES) are algorithms derived from Evolutionary Algorithms (EA), based on the application of mutation, recombination and selection in populations of candidate solutions \cite{hansen2015}.
The table \ref{tab_basicES} below, summarizes the main elements of Evolution Strategies. 
\begin{table}[htbp]
\caption{Basic Elements of Evolution Strategies \cite{EibenS03}}
\begin{center}
\label{t1}
\begin{tabular}{p{0.3\linewidth} | p{0.5\linewidth}}
 \hline
 Representation & Real-valued vectors \\
\hline
 Recombination & Discrete or intermediary \\
\hline
Mutation & Gaussian perturbation\\
\hline
Parent selection & Uniform random \\
\hline
Survivor selection & Deterministic elitist replacement by $\mu , \lambda$ or $\mu + \lambda$\\
\hline
Speciality &Self-adaptation of mutation step sizes\\
\hline
\end{tabular}
\label{tab_basicES}
\end{center}
\end{table}

\noindent Many real-world application problems can be formulated to optimize an objective function $min_{x\in\Omega}f(x)$, where $\Omega \subset \mathbf{R}^n$ is the search space, and $x$ is the decision variable. Black-box optimization refers to the scenarios that the analytical expression and gradient of the objective function $f$ are unavailable, and the only information accessible is the objective value for any given point $x\in\Omega$. ES can therefore be leveraged for black-box optimization and achieve state-of-the-art performance on many benchmarks and real-world  applications \cite{Zhenhua2020,hansen2015}.\\
The framework for evolution Strategies is presented in both figure \ref{fig_ES} and \ref{fig_ev} and below.\\
\begin{figure}[t]
\centerline{\includegraphics[width=\columnwidth]{images/evolution.png}}
\caption{The general scheme of Evolution Algorithms \cite{EibenS03}}
\label{fig_ev}
\end{figure}

\begin{figure*}[t]
\centerline{\includegraphics[width=5.5in]{images/ES_fig.png}}
\caption{Overall Evolution Strategies}
\label{fig_ES}
\end{figure*}
\noindent ES can be defined as an algorithm providing a user with a set of candidate solutions for evaluating a specific problem. The steps are as follows \cite{Khan2008,Zhenhua2020,EibenS03}:
\begin{itemize}
    \item The first step consists of generating a random population P of individuals.
    Each individual consists of a solution and an associated fitness value, $f(x)$, and can be denoted as a parent individual.
    \item In the recombination step, parent individuals are chosen and their respective values are recombined to produce offspring individuals (this is done by either taking average values or by exchanging randomly chosen components of the parent pair). Gaussian noise is then added to the solutions in the mutation step, allowing for stochastic exploration of the design space.
    \item The next step consists of evaluating the individuals’ fitnesses $f(x)$.
    \item Only the best individuals from the population survive and are chosen as parent individuals for the next generation.
    \item This process then continues and repeats until a stop condition is met.
\end{itemize}
Evolution strategies therefore usually evolve a Gaussian distribution to search promising solutions for the objective function . In the general case, the search distribution is parameterized by $N(m,\sigma^2C)$ where:
\begin{itemize}
    \item $m$: the mean $m$ determines the center of the search distribution and
    represents the favorable solution.
    \item $C$: the covariance matrix determines the shape of the underlying distribution.
    It gradually represents the correlations between variables and the relative scalings along different directions.
    \item $\sigma$: the global variance $\sigma$ is a scale factor that determines the length
    along any direction. It can be termed step size or mutation strength. The step size enables the distribution to approach the optimum rapidly without careful adaptation of the covariance matrix.
\end{itemize}

\noindent Throughout this paper, Evolutionary Strategies are differentiated from Genetic Algorithms. Table \ref{t1} identifies the main differences between GAs and ESs \cite{HoffmeisterB90}.
\begin{table}[htbp]
\caption{Evolution Strategies vs Genetic Algorithms}
\begin{center}
\label{t1}
\begin{tabular}{p{0.4\linewidth} | p{0.4\linewidth}}
 \hline 
 Evolutionary Strategies & Genetic Algorithms \\
 \hline\hline
 Phenotype level of individuals (real-valued representation) & Genotype level of individuals (binary coding) \\ 
  \hline
 Knowledge of the dimension of the objective function (i.e. number of variables) & No knowledge about the properties of the objective function \\
  \hline
 No parameter restrictions apart from machine-dependencies & Parameter space restrictions for decoding purposes  \\
  \hline
 $(\mu,\lambda)$-selection and $(\mu+\lambda)$-selection & Proportional selection and Ranking \\
  \hline
 Mutation serves as the main search operator  & Recombination serves as the main search operator \\ 
   \hline
 Several recombination schemes & Secondary role of mutation  \\
   \hline
 Collective self-learning of strategy parameters& No collective self-learning of parameter settings  \\
 \hline
\end{tabular}
\label{tab1}
\end{center}
\end{table}\\

% \noindent ES is very similar to other policy search algorithms:
% \begin{itemize}
%   \item you have a neural network that represents the policy, i.e. a function that decides what action to take given the current state
%   \item you need to improve this policy so that the total reward is maximized
% \end{itemize}
% The difference is in how you improve the policy. While other RL methods explore the action world by trying different random actions and essentially reinforce the good ones, ES works directly on the parameters of the network and randomly jitters them around hoping to find good outcomes. When using ESs, we do not need to know anything about how the policy works. It is a box with an input (state) and output (actions) and we move around the knobs (weights) until we find a better solution, hopefully the optimal solution.
% Given an initial policy (either random or pre-learned through supervised learning) we can always generate a population of similar policies around it by applying random perturbations to its weights. We then evaluate all these new policies and estimate the gradient, that is, we check in what direction things look more promising. Finally, we update the initial weights to move exactly in that direction and start again from there. We loop until we are happy with the outcome.

% \begin{figure}[htbp]
% \centerline{\includegraphics[width=\columnwidth]{images/ES_path.png}}
% \caption{Evolution follows the best path \cite{Deepanshu2020}}
% \label{ES_path}
% \end{figure}

% Figure \ref{ES_path} shows that given an initial policy, we can always generate a population of similar policies around it by applying random changes to its weights. We then evaluate all these new policies and estimate the gradient i.e. we check in what direction things look more promising. Finally, we update weights and policy parameters to move exactly in that direction and start again and loop until we are satisfied with the outcome.\cite{Deepanshu2020}

\textbf{\textit{Common algorithms.}} This section will go over the main ES algorithms, giving a high level overview of how each works.

\noindent \textit{Covariance Matrix Adaptation Evolution Strategies (CMA-ES).} CMA-ES was first defined by Hansen et al. \cite{hansen2016cma}, and is one of the most popular gradient-free optimisation algorithms, and has been the algorithm of choice for many researchers.  CMA-ES is an algorithm that will take the output of each generation and increase or decrease the search space accordingly for the next generation.The latter adaptation allows CMA-ES to optimize the search space by either increasing it when the best solutions are far away, or narrowing it when the best solutions are close by. At each different generation, CMA-ES samples the solutions from the parameters of a multi-variate normal distribution. CMA-ES has one main drawback relating to its performance decrease in case the number of model parameters to solve for is large. 
The basic idea behind CMA-ES is shown in the steps below and in Figure \ref{fig_CMAES}:
\begin{enumerate}
  \item Calculate the fitness score of each candidate solution in generation (g)
  \item Isolates the best X\% of the population in generation (g)
  \item Using only the best solutions, along with the mean $\mu^{(g)}$ of the current generation calculate the covariance matrix $C^{(g+1)}$ of the next generation.  
  \item Sample a new set of candidate solutions using the updated mean $\mu^{(g+1)}$ and covariance matrix $C^{(g+1)}$
\end{enumerate}
\begin{figure}[htbp]
\centerline{\includegraphics[width=4in]{images/cmaes.png}}
\caption{Covariance Matrix Adaptation Evolution Strategies (CMA-ES) \remark{try to recreate this using the algorithm I found}}
\label{fig_CMAES}
\end{figure}
 While being one of the most efficient ESs, CMA-ES had still proven to be unsuitable for large scale optimization and also unsuited to the training of deep neural networks and the solving of deep RL problems \cite{ijcai2019} \cite{Varelas2018}. When training neural networks, CMA-ES needs much more time to keep track and revise its full covariance matrix, due to its quadratic time complexity. As a result, the research of applying CMA-ES to RL still has some gaps. \\
% In \cite{Verena2008}, a comparison was made between two general approaches to conduct direct policy search (as seen in Figure \ref{fig1}) for reinforcement learning: policy gradient methods (PGMs) and evolution strategies (ESs). Verena et al. \cite{Verena2008} thus compares between a Reinforcement Learning algorithm: the natural actor critic algorithm (NAC) and an Evolution Strategy one: covariance matrix adaptation ES (CMA-ES). Both these implementations are compared in an attempt to point out their similarities and differences as both can be utilized in the policy search process when mapping the states to the actions an agent can take, all the while optimizing future reward. Both types of algorithms mainly perform the same steps to obtain a solution. They differ however in the order of these steps and the level at which the random changes are applied. A series of experiments based on the "pole-balancing" problem in RL are performed in which CMA-ES seemed more robust as relating to the choice of hyperparameters and initial policies. In terms of learning speed, the natural policy gradient ascent performs similarly as CMA-ES for fine-tuning and may even be desirable in some cases.\\
% \noindent A more recent research on CMA-ES as a replacement for Reinforcement learning was also performed in "Robot Skill Learning: From Reinforcement Learning to Evolution Strategies" \cite{stulp2013}.In their paper, Stulp et al. showcase that reinforcement learning (RL) algorithms have become more and more similar to evolution strategies such as $(\mu_w , \lambda)-ES$ and CMA-ES. The authors thus give an overview of several policy improvement algorithms, and demonstrate that these methods are getting closer and closer to Evolution Strategies as Evolution strategies also use parameter space exploration and reward-weighted averaging. ES do however treat policy improvement as a black-box optimization (BBO) problem.  Stulp et al. therefore close the gap between RL and BBO tasks, by showcasing that two simplification in the state-of-the-art PI2 RL algorithm are enough for converting it into the evolutionary strategy $(\mu_w , \lambda)-ES$, a BBO algorithm in which CMA-ES is rooted. Moreover in \cite{stulp2013}, the authors observe that $(\mu_w , \lambda)-ES$, is able to outperform state-of-the-art policy improvement algorithms such as PI2 and PoWER with policy representations commonly considered in the robotics field.\\%not relly the best. for big probllems in rL \\
% A restart-based rank-1 evolution strategy (called R-R1-ES for short) for RL \cite{chen2019restart} was also proposed in 2019 and can be regarded as a simplified CMA-ES. It can retain the excellent performance of CMA-ES. It has a linear time and low space complexity, thus making it fit for dealing with large scale black-box optimization and deep RL problems. As in other algorithms derived after the release of OpenAI-ES, \cite{salimans2017evolution}, the technique of virtual batch normalization and other reparameterizations of the neural network policy are adopted to enhance the reliability of R-R1-ES. Moreover, by leveraging the parallelization aspect of ES, a novel communication strategy based on common random numbers is introduced to reduce communication cost, allowing the algorithm to properly scale for a large number of parallel workers. Experimental results on classic control problems and Atari games show that the proposed algorithm \cite{chen2019restart} is superior to or competitive with state-of-the-art algorithms for reinforcement learning, demonstrating its effectiveness.\\
\noindent \textit{Natural Evolution Strategies (NES).} NES algorithms iteratively update a search distribution by using an estimated gradient on the distribution parameters \cite{Wierstra2014}. The main steps included for NES are:
\begin{itemize}
  \item The parameterized search distribution is used to produce a batch of search points on which the fitness function will be evaluated.
  \item The distribution’s parameters (including strategy parameters) allow the algorithm to adaptively capture the  structure of the fitness function.
  \item From the samples computed, NES estimates a search gradient on the parameters towards higher expected fitness.
  \item NES then performs a gradient ascent step along the natural gradient, renormalizing the update with respect to uncertainty. This will prevent oscillations, premature convergence, and undesired effects from a given parameterization.
  \item The entire process reiterates until a stopping criterion is met. \cite{Wierstra2014}
\end{itemize}

As of late, several of these ES algorithms are being considered as alternatives for RL. The algorithms presented below are thus extracted from the literature and showcase the use of ES methods for RL tasks.\\
\noindent \textit{OpenAI-ES.} A third identified Evolution Strategy, is OpenAI-ES. In \cite{salimans2017evolution}, Salimans et al. implemented an evolution strategy that is a simplified special case of the NES algorithm outlined earlier. In particular, $\sigma$ is fixed to a constant number, and only the $\mu$ parameter is updated at each generation. Throughout their paper, Salimans et al. proposed a modification of the update rule that is suitable for parallel computation across different worker machines.This new update rule thus consists of holding a large grid of random numbers which have been pre-computed using a fixed seed. Each worker can then reproduce the parameters of every other worker over time, and each worker needs only to communicate a single number, the final fitness result, to all of the other workers, thus limiting the transmission of an entire solution vector a million times at each generation update which may be unfeasible. The latter allows for scaling evolution strategies to thousands or even a million workers located on different machines. 
The paper by Saliman et al. \cite{salimans2017evolution} opened the doors to many researchers for discussing the competitive aspect of ES, its potential improvements and combination with RL algorithms.\\
\begin{figure}[htbp]
\centerline{\includegraphics[width=3.60in]{images/openAI.png}}
\caption{OpenAI Evolution Strategy (OpenAI-ES) \remark{try to recreate this }}
\label{fig_CMAES}
\end{figure}
\noindent\textit{R-R1-ES. }A restart-based rank-1 evolution strategy (called R-R1-ES for short) for RL \cite{chen2019restart} was also proposed in 2019 and can be regarded as a simplified CMA-ES. It can retain the excellent performance of CMA-ES. It has a linear time and low space complexity, thus making it fit for dealing with large scale black-box optimization and deep RL problems. As in other algorithms derived after the release of OpenAI-ES, \cite{salimans2017evolution}, the technique of virtual batch normalization and other reparameterizations of the neural network policy are adopted to enhance the reliability of R-R1-ES. Moreover, by leveraging the parallelization aspect of ES, a novel communication strategy based on common random numbers is introduced to reduce communication cost, allowing the algorithm to properly scale for a large number of parallel workers. Experimental results on classic control problems and Atari games show that the proposed algorithm \cite{chen2019restart} is superior to or competitive with state-of-the-art algorithms for reinforcement learning, demonstrating its effectiveness.\\
\noindent \textit{Canonical ES algorithm.} Having explored ES algorithms that belonged to the specialized class of natural evolution strategies, several researchers were interested in demonstrating that even very a basic canonical ES algorithm can achieve the same or even better performance than the OpenAI-ES algorithm. Chrabaszcz et al. \cite{chrabaszcz2018basics} thus showed that a variation of the simple $(\mu; \lambda)-ES$ algorithms,can be used for tasks which are now dominated by reinforcement learning (RL).  This algorithm is very basic and simpler than the NES-rooted algorithm by Salimans et al. \cite{salimans2017evolution}. The enhancements made known by Salimans et al. \cite{salimans2017evolution} such as  virtual batch normalization and the parallelization of ES using a random noise table were both leveraged by Chrabaszcz et al. \cite{chrabaszcz2018basics}, thus showing that OpenAI-ES acted as a precursor for other works. Chrabaszcz et al. therefore demonstrated that Canonical ES is a competitive alternative to traditional RL algorithms and to the previously proposed ES algorithms tested so far on the Atari games \cite{chrabaszcz2018basics} \cite{salimans2017evolution}. Seeing how the canonical ES version appears to be a viable alternative, it can be considered as a basis for future work on more modern ES variants, as it shows that state-of-the-art algorithms can be taken even further by leveraging the advances made in the field of ES in the last decades.\\
%\subsubsection{Natural evolution strategy (NES) approach}\hspace*{\fill} \\
% While research on Evolution Strategies and of their use for free gradient policy computation is no new topic per say, it is not until a few years back that the benefits of these methods were showcased as a viable alternative to Reinforcement Learning. Salimans et al. \cite{salimans2017evolution} thus explored in 2017 the feasibility of using Evolutionary Strategies from the class of Natural Evolution Strategies for training a deep neural network as compared to using a more conventional Reinforcement Learning method using back-propagation such as Q-learning and Policy gradients. Usually neural networks are trained using back-propagation to update the weights. When applied to Reinforcement Learning, the neural network explores different actions in the environment and these actions return values used to update the weights of the network. This can be considered searching in the action space. ES searches for the best weights of the network where the environment is a black-box that returns a score on the performance of any particular set of parameters. This is known as searching the parameter space.\\
%\subsubsection{covariance matrix evolution strategy (CMA-ES) approach}\hspace*{\fill} \\


%\subsubsection{Canonical evolution strategy (C-ES) approach}\hspace*{\fill} \\
% Having explored ES algorithms that belonged to the specialized class of natural evolution strategies, several researchers were interested in demonstrating that even very a basic canonical ES algorithm can achieve the same or even better performance than the OpenAI-ES algorithm. Chrabaszcz et al. \cite{chrabaszcz2018basics} thus showed that a variation of the simple $(\mu; \lambda)-ES$ algorithms,can be used for tasks which are now dominated by reinforcement learning (RL).  This algorithm is very basic and simpler than the NES-rooted algorithm by Salimans et al. \cite{salimans2017evolution}. The enhancements made known by Salimans et al. \cite{salimans2017evolution} such as  virtual batch normalization and the parallelization of ES using a random noise table were both leveraged by Chrabaszcz et al. \cite{chrabaszcz2018basics}, thus showing that OpenAI-ES acted as a precursor for other works. Chrabaszcz et al. therefore demonstrated that Canonical ES is a competitive alternative to traditional RL algorithms and to the previously proposed ES algorithms tested so far on the Atari games \cite{chrabaszcz2018basics} \cite{salimans2017evolution}. Seeing how the canonical ES version appears to be a viable alternative, it can be considered as a basis for future work on more modern ES variants, as it shows that state-of-the-art algorithms can be taken even further by leveraging the advances made in the field of ES in the last decades.\\

==> sections/draft/draft.tex <==
Policy search methods usually use either gradient-based or gradient-free optimization, and both can successfully train neural networks that encode policies. Gradient-free optimization can effectively cover low-dimensional parameter
spaces, but, despite some successes in applying them to large networks, gradient-based training remains the method of
choice for most DRL algorithms, being more sample efficient when policies possess a large number of parameters.
With gradient-free methods, finding better policies requires a heuristic search across a predefined class of models. Methods such as Evolution strategies thus come into play.\\

The   ”Covariance   Matrix   Adaptation   Evolution   Strategies(CMA-ES)”  is proposed throughout the literature for solving reinforcement learning tasks. In \cite{Verena2008}, a comparison is thus made between two general approaches to conduct direct policy search for reinforcement learning: policy gradient methods (PGMs) and evolution strategies (ESs). Verena et al. \cite{Verena2008} thus compares between a Reinforcement Learning algorithm: the natural actor critic algorithm (NAC) and an Evolution Strategy one: covariance matrix adaptation ES (CMA-ES). Both these implementations are thus compared in an attempt to point out their conceptual
similarities and differences as both can be leveraged in the search for a policy mapping states of the environment to the actions an agent can take in those states, in an effort to maximize future reward. As seen in Figure \ref{comparison}, both types of algorithms perform the same conceptual steps to obtain the solution. They differ in the order of these steps and the level at which the random changes are applied. A series of experiments based on the "pole-balancing" problem in RL were thus performed. The latter showed that CMA-ES is more robust w.r.t. to the choice of
hyperparameters and initial policies. In terms of learning speed, the natural policy gradient ascent performs on par for fine-tuning and may be preferable in this scenario.\\
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/policy.PNG}
    \caption{Conceptual similarities and differences
of natural policy gradient ascent and CMA
evolution strategy: Both methods adapt a
metric for the variation of the policy parameters
based on information received from the
environment. Both explore by stochastic perturbation
of policies, but at different levels. by Verena et al. \cite{Verena2008}}
    \label{comparison}
\end{figure}
A more recent research on CMA-ES as a replacement for Reinforcement learning was also performed in "Robot Skill Learning: From Reinforcement Learning to Evolution Strategies" \cite{stulp2013}.In their paper, Stulp et al. showcase that reinforcement learning (RL) algorithms have become more and more similar to evolution strategies such as $(\mu_w , \lambda)-ES$ and CMA-ES. The authors thus give an overview of several policy improvement algorithms,
and demonstrate that a side-effect of these trends has been
that they have brought these algorithms closer and closer to evolution strategies such as CMA-ES. Evolution strategies also use parameter space exploration and reward-weighted averaging, but treat policy improvement as a black-box optimization (BBO) problem, and thus do not leverage the problem structure, whereas RL algorithms do. They draw a strong bridge between RL and BBO, by showing that only two straightforward simplifications suffice to convert the state-of-the-art PI2 RL algorithm into the evolutionary strategy $(\mu_w , \lambda)-ES$, a BBO algorithm which is the backbone of CMA-ES, and make a rather surprising observation: $(\mu_w , \lambda)-ES$– one of the most basic evolution strategies – is able to outperform state-of-the-art policy improvement algorithms such as PI2 and PoWER with policy representations typically considered in the robotics community.\\%not relly the best. for big probllems in rL \\

In their paper "Evolution Strategies as a Scalable Alternative to Reinforcement Learning" \cite{salimans2017evolution} , Salimans et al. explore the feasibility of using Evolutionary Strategies for training a deep neural network as compared to using a more conventional Reinforcement Learning method which leverages back-propagation such as Q-learning and Policy gradients. Usually neural networks are trained using back-propagation to update the weights. When applied to Reinforcement Learning, the neural network explores different actions in the environment and these actions return values which is used to update the weights of the network. This can be considered searching in the action space. ES searches for the best weights of the network where the environment is a black-box that returns a score on the performance of any particular set of parameters. This is known as searching the parameter space.\\
ES is thus a black box optimization method which leverages capabilities from both Random Search algorithms and evolutionary algorithms in hopes of finding the optimumum parameters $\theta$ for training a deep neural network.\\
The great benefit of this approach is that it is parallelizable with little effort. Whereas RL methods such as A3C need to communicate gradients back and forth between workers and a parameter server, ES only requires fitness scores and high-level parameter distribution information to be communicated. It is this simplicity that allows the technique to scale up in ways current RL methods cannot. All of this comes at a cost however: the cost of treating the network being optimized as a black-box. By black-box, I mean that the inner workings of the network are ignored in the training process, and only the overall outcome (episode-level reward) is utilized in determining whether to propagate the specific network weights to further generations. In situations where we don’t get a strong feedback signal from the environment, such as many traditionally posed RL problems with only sparse rewards, turning the problem from a “mostly black box” into an “entirely black box” is worth the performance improvements that can come along with it.\\
Seeing how ES is defined as easily parallelizable, Salimans et al.'s approach consists of maintaining a distribution over network weight values, and having a large number of agents act in parallel using parameters sampled from this distribution. Each agent acts in its own environment, and once it finishes a set number of episodes, or steps of an episode, cumulative reward is returned to the algorithm as a fitness score. With this score, the parameter distribution can be moved toward that of the more successful agents, and away from that of the unsuccessful ones. By repeating this approach millions of times, with hundreds of agents, the weight distribution moves to a space that provides the agents with a good policy for solving the task at hand. \\
The researchers applied ES to MuJoCo (continuous robotic control, eg walking/hopping/swimming) tasks and several Atari games. ES was able to solve the MuJoCo tasks and performed competitively on the Atari games. Matching the network architecture and level of computation presented in the paper Asynchronous Methods for Deep Reinforcement Learning, ES performed better in 23 games and worse in 28. Due to parallelization, it was possible to solve the 3D Humanoid walking task in just ten minutes using 1440 CPU cores.\\
In "On the Relationship Between the OpenAI Evolution Strategy and Stochastic Gradient Descent" \cite{zhang2017relationship}, Zhang et al. \\

In the paper "Back to Basics: Benchmarking Canonical Evolution Strategies for Playing Atari" \cite{chrabaszcz2018basics}, Chrabaszcz et al. that even a very basic canonical ES algorithm can achieve the same or even better performance than the OpenAI's ES algorithm. This success of a basic
ES algorithm suggests that the state-of-the-art can be advanced further by integrating the many advances made in the field of ES in the last decades. We also demonstrate qualitatively that ES algorithms have very different performance characteristics than traditional RL algorithms: on some games, they learn to exploit the environment and perform much better while on others they can get stuck in suboptimal local minima. Combining their strengths with those of traditional RL algorithms is therefore likely to lead to new advances in the state of the art.\\


%Talk about Back to Basics: Benchmarking Canonical Evolution Strategies for Playing Atari
%So ES: CMAES, basic and NES we have papers for all 3
%COmpare to RL
%Talk about Challenges in High-dimensional Reinforcement Learning with Evolution Strategies
\subsection{Comparing Deep reinforcement learning and Evolution Strategies}

In the paper "Comparing Deep Reinforcement Learning and Evolutionary Methods in Continuous Control" by Zhang et al. \cite{zhang2018comparing}, the authors present a comprehensive  comparison between Deep Reinforcement Learning and Evolutionary Methods as applied to complex continuous control tasks. It aims to understand the advantages and disadvantages of both methods in order to properly assess the use of each, focusing on control problems.\\
Continuous control systems such as robotics control are challenging for both RL and ES methods. Throughout this paper, the authors considered the CA3C, P3O and D3PG algorithms as the representatives of the state-of-the-art deep RL methods, and CMAES, NEAT and NES as the representatives of the state of art evolutionary methods. Each of the algorithms is therefore first explained in the paper before actually getting to the comparison. The algorithms are implemented in a parallelized manner across multiple processes and comparison was conducted in terms of wall time and environment time steps. 
For the experimentation, various testbeds were considered: Pendulum task, Continuous Lunar Lander task, the Bipedal Walker task and the Bipedal Waler Hardcore task. We can hardly say which algorithm is the best, as no algorithm can consistently outperform others across all the tasks. NEAT achieved a good performance level in the three Box2D tasks, but failed the simplest Pendulum task. One interesting observation is that all the evolutionary methods solved the Continuous Lunar Lander task, but most deep RL methods appeared to get trapped in some local minima, which denotes that evolutionary methods are better at exploration than the deep RL methods. However when it comes to the two Walker tasks, where rich dynamics are involved, most deep RL methods worked better and the evolutionary methods appeared to get trapped in some local minima, which denotes that the deep RL methods can handle rich dynamics better than the evolutionary methods. In terms of data efficiency, the deep RL methods can solve tasks with much less interaction with the environment than the evolutionary methods, and the wall time is usually shorter, at worst comparable. In conclusion, the performance of the parallelized algorithms appears to be task dependent. But in general, NEAT, D3PG and P3O are safe choices. \\
Salimans et al.\cite{salimans2017evolution} thus lists the advantages of his approach. ES thus seems to add many advantages to RL algorithms. It removes the need for backpropagation. ES only requires the forward pass of the policy and does not require backpropagation (or value function estimation), which makes the code shorter and between 2-3 times faster in practice. On memory-constrained systems, it is also not necessary to keep a record of the episodes for a later update. There is also no need to worry about exploding gradients in RNNs. Lastly, we can explore a much larger function class of policies. Moreover, ES methods are highly parallelizable. ES only requires workers to communicate a few scalars between each other, while in the more standard RL it is necessary to synchronize entire parameter vectors (which can be millions of numbers). Intuitively, this is because we control the random seeds on each worker, so each worker can locally reconstruct the perturbations of the other workers. Thus, all that we need to communicate between workers is the reward of each perturbation. As a result, we observed linear speedups in our experiments as we added on the order of thousands of CPU cores to the optimization.Additionally ES provides higher robustness. Several hyperparameters that are difficult to set in RL implementations are side-stepped in ES. For example, RL is not “scale-free”, so one can achieve very different learning outcomes (including a complete failure) with different settings of the frame-skip hyperparameter in Atari. As we show in our work, ES works about equally well with any frame-skip. ES also gives access to structured exploration. Some RL algorithms (especially policy gradients) initialize with random policies, which often manifests as random jitter on spot for a long time. This effect is mitigated in Q-Learning due to epsilon-greedy policies, where the max operation can cause the agents to perform some consistent action for a while (e.g. holding down a left arrow). This is more likely to do something in a game than if the agent jitters on spot, as is the case with policy gradients. Similar to Q-learning, ES does not suffer from these problems because we can use deterministic policies and achieve consistent exploration. \\
In the paper "Challenges in High-dimensional Reinforcement Learning
with Evolution Strategies", \cite{muller2018challenges} investigated the utility of diferent algorithmic mechanisms of evolution strategies
for problems with a specic combination of challenges, namely high-dimensional search spaces
and tness noise.

Efficacy of Modern Neuro-Evolutionary Strategies for Continuous Control Optimization
%Evolution Strategies as a Scalable Alternative to Reinforcement Learning
%Similarities and differences between policy gradient methods and evolution strategies
%ES Is More Than Just a Traditional Finite-Difference Approximator
%Robot Skill Learning: From Reinforcement Learning to Evolution Strategies
%Deep Neuroevolution: Genetic Algorithms are a Competitive Alternative for Training Deep Neural Networks for Reinforcement Learning
%Comparing Deep Reinforcement Learning and Evolutionary Methods in Continuous Control
%Back to Basics: Benchmarking Canonical Evolution Strategies for Playing Atari
\begin{table}[htbp]
\caption{Evolution Strategies vs Genetic Algorithms}
\begin{center}
\label{t1}
\begin{tabular}{l l l}
 \hline 
   & Evolutionary Strategies & Genetic Algorithms \\
 \hline\hline
 Initial Population & Random mutations & Random or seeded \\ 
%  \hline
 Evaluation & Objective function & Fitness function \\
%  \hline
 Selection & Truncation selection & Different methods  \\
%  \hline
 Reproduction & Recombination + Mutation & Crossover + Mutation \\
%  \hline
 Termination & User dependent & User dependent \\ 
 \hline
\end{tabular}
\label{tab1}
\end{center}
\end{table}

==> sections/draft/fromRLtoES.tex <==
Evolution Strategies can therefore be used to train a neural network without back propagation. Throughout this section, we will show how  Evolution Strategies can be easily implemented in a Reinforcement learning setup and showcase their scalability in a distributed computational environment. 

\subsection{Evolutionary Strategies as part of Reinforcement Learning}

Deep artificial neural networks (DNNs) are typically trained via gradient-based learning algorithms, namely backpropagation. Evolution
strategies (ES) can rival backprop-based algorithms such as Q-learning and policy gradients
on challenging deep reinforcement learning (RL) problems

In their paper "Evolution Strategies as a Scalable Alternative to Reinforcement Learning", Salimans et al. explore the feasibility of using Evolutionary Strategies for training a deep neural network as compared to using a more conventional Reinforcement Learning method which leverages back-propagation such as Q-learning and Policy gradients. Usually neural networks are trained using back-propagation to update the weights. When applied to Reinforcement Learning, the neural network explores different actions in the environment and these actions return values which is used to update the weights of the network. This can be considered searching in the action space. ES searches for the best weights of the network where the environment is a black-box that returns a score on the performance of any particular set of parameters. This is known as searching the parameter space.\\
ES is thus a black box optimization method which leverages capabilities from both Random Search algorithms and evolutionary algorithms in hopes of finding the optimumum parameters $\theta$ for training a deep neural network.\\
Evolutionary Strategies act as a black box optimization aolgorithm, aiming to maximize the return function $F(\theta)$ with respect to $\theta$. The OpenAI Evolutionary Statretgy method is therefore based on the Natural Evolution Strategy paradigm and acts on the idea of "finite differences" . Imagine having a function $F(\theta)$ which creates a neural network with weights $\theta$, run the neural network on the environment for some time, sum up and return the total reward. Considering now that our function acts as a black box, and that we can only perceive the parameters going in and those coming out, the proposed Evolutionary Strategies implementation would first sample points (potential weights) by starting with some random parameter vector, and generate a popluation of various otehr parameter vectors $\theta_1....\theta_100$ by jittering $\theta$ with gaussian noise. The different vecotrs will then be evaluated on the function and their respective rewards will be computed. The updated parameter vector then becomes the weighted sum of the different vectors, where each weight is proportional to the total reward (i.e. we want the more successful candidates to have a higher weight). In this way, the new ‘best’ will move in the direction that maximizes performance and reward in the environment. \\
The great benefit of this approach is that it is parallelizable with little effort. Whereas RL methods such as A3C need to communicate gradients back and forth between workers and a parameter server, ES only requires fitness scores and high-level parameter distribution information to be communicated. It is this simplicity that allows the technique to scale up in ways current RL methods cannot. All of this comes at a cost however: the cost of treating the network being optimized as a black-box. By black-box, I mean that the inner workings of the network are ignored in the training process, and only the overall outcome (episode-level reward) is utilized in determining whether to propagate the specific network weights to further generations. In situations where we don’t get a strong feedback signal from the environment, such as many traditionally posed RL problems with only sparse rewards, turning the problem from a “mostly black box” into an “entirely black box” is worth the performance improvements that can come along with it.\\
Seeing how ES is defined as easily parallelizable, Salimans et al.'s approach consists of maintaining a distribution over network weight values, and having a large number of agents act in parallel using parameters sampled from this distribution. Each agent acts in its own environment, and once it finishes a set number of episodes, or steps of an episode, cumulative reward is returned to the algorithm as a fitness score. With this score, the parameter distribution can be moved toward that of the more successful agents, and away from that of the unsuccessful ones. By repeating this approach millions of times, with hundreds of agents, the weight distribution moves to a space that provides the agents with a good policy for solving the task at hand. \\
The researchers applied ES to MuJoCo (continuous robotic control, eg walking/hopping/swimming) tasks and several Atari games. ES was able to solve the MuJoCo tasks and performed competitively on the Atari games. Matching the network architecture and level of computation presented in the paper Asynchronous Methods for Deep Reinforcement Learning, ES performed better in 23 games and worse in 28. Due to parallelization, it was possible to solve the 3D Humanoid walking task in just ten minutes using 1440 CPU cores.\\
Based on the results from this paper, ES thus seems to add many advantages to RL algorithms. It removes the need for backpropagation. ES only requires the forward pass of the policy and does not require backpropagation (or value function estimation), which makes the code shorter and between 2-3 times faster in practice. On memory-constrained systems, it is also not necessary to keep a record of the episodes for a later update. There is also no need to worry about exploding gradients in RNNs. Lastly, we can explore a much larger function class of policies. Moreover, ES methods are highly parallelizable. ES only requires workers to communicate a few scalars between each other, while in the more standard RL it is necessary to synchronize entire parameter vectors (which can be millions of numbers). Intuitively, this is because we control the random seeds on each worker, so each worker can locally reconstruct the perturbations of the other workers. Thus, all that we need to communicate between workers is the reward of each perturbation. As a result, we observed linear speedups in our experiments as we added on the order of thousands of CPU cores to the optimization.Additionally ES provides higher robustness. Several hyperparameters that are difficult to set in RL implementations are side-stepped in ES. For example, RL is not “scale-free”, so one can achieve very different learning outcomes (including a complete failure) with different settings of the frame-skip hyperparameter in Atari. As we show in our work, ES works about equally well with any frame-skip. ES also gives access to structured exploration. Some RL algorithms (especially policy gradients) initialize with random policies, which often manifests as random jitter on spot for a long time. This effect is mitigated in Q-Learning due to epsilon-greedy policies, where the max operation can cause the agents to perform some consistent action for a while (e.g. holding down a left arrow). This is more likely to do something in a game than if the agent jitters on spot, as is the case with policy gradients. Similar to Q-learning, ES does not suffer from these problems because we can use deterministic policies and achieve consistent exploration. 
Calling this paper an alternative to RL can thus be considered as a mistake and it should be called rather alternative to back propagation. the title is somewhat misleading. What they are doing is still RL. They have a parameterized policy, and they utilize ES instead of policy gradient to update the policy network weights. In terms of performance, it's indeed faster in absolute clock time compared to policy gradient, due to the ability to parallelize a large population of policy weights for roll-outs. But its still less efficient sample wise (total of # of roll-outs needed).\\
One more point, everything looks good so far since most RL results are run in simulated worlds. The kind of high parallelism required by ES would be much harder to replicate if your applying it to say real life robotics applications. But this would be an important thing to think abut when doing swarm robots with multiple robots able to think together. It would therefore be possible to omplement these algorithms in a parallel
distributed fashion for learning in multi-robot systems.  Eachrobot is responsible for several virtual agents, which it evaluates at each iteration. After each set of evaluations, the robots communicate to share the fitness information needed to progress to the next iteration of the algorithm. By running the algorithms in this fashion, we need no external supervisor to oversee the learning process, and the speed of learning is significantly improved, as many robots evaluating in parallel increase the rate of candidate solution evaluation
and therefore decrease the total learning time.
%Parallel Learning in Heterogeneous Multi-Robot Swarms
%Jim Pugh, Member, IEEE and Alcherio Martinoli, Member, IEEE

In the paper "Comparing Deep Reinforcement Learning and Evolutionary Methods in Continuous Control" by Zhang et al., the authors present a comprehensive  comparison between Deep Reinforcement Learning and Evolutionary Methods as applied to complex continuous control tasks. It aims to understand the advantages and disadvantages of both methods in order to properly assess the use of each, focusing on control problems.\\
Continuous control systems such as robotics control are challenging for both RL and ES methods. Throughout this paper, the authors considered the CA3C, P3O and
D3PG algorithms as the representatives of the state-of-the-art deep RL methods, and CMAES, NEAT and NES as the representatives of the state of art evolutionary methods. Each of the algorithms is therefore first explained in the paper before actually getting to the comparison. The algorithms are implemented in a parallelized manner across multiple processes and comparison was conducted in terms of wall time and environment time steps. 
For the experimentation, various testbeds were considered: Pendulum task, Continuous Lunar Lander task, the Bipedal Walker task and the Bipedal Waler Hardcore task. We can hardly say which algorithm is the best, as no algorithm can consistently outperform others across all the tasks. NEAT achieved a good performance level in the three Box2D tasks, but failed
the simplest Pendulum task. One interesting observation is that all the evolutionary methods solved the Continuous Lunar Lander task, but most deep RL methods appeared to get trapped in some local minima, which denotes that evolutionary methods are better at exploration than the deep RL methods. However when it comes to the two Walker tasks, where rich dynamics are involved, most deep RL methods worked better and the evolutionary methods appeared to get trapped in some local minima, which denotes that the deep RL methods can handle rich dynamics better than the evolutionary methods. In terms of data efficiency, the deep RL methods can solve tasks with much less interaction with the environment than the evolutionary methods, and the wall time is usually shorter, at worst comparable. In conclusion, the performance of the parallelized algorithms appears to be task dependent. But in general, NEAT, D3PG and P3O are safe choices. 

\subsection{Improving on Evolutionary Strategies}
In the paper "Improving Exploration in Evolution Strategies for Deep Reinforcement Learning via a Population of
Novelty-Seeking Agents", Conti et al. introduces new scalable algorithms for reinforcement learning that 
are capable of directed exploration. Algorithms such as novelty search (NS) and quality diversity
(QD) are thus  hybridized with ES to improve its performance on sparse or deceptive deep RL tasks, while retaining scalability. The authors thus first study NS, which performs exploration only (ignoring the reward function) to find a set of novel solutions before investigating algorithms that balance exploration and exploitation, specifically novel instances of QD algorithms.\\
As previously mentioned in "Evolution  Strategies  as  a  Scalable  Alter-native  to  Reinforcement  Learning", 
ES directly searches in the parameter space of a neural network to find an effective policy. Salimans et al. has thus shown that  ES can achieve competitive performance on many reinforcement learning (RL) tasks due to it being highly parallelizable, which enables near linear speedups in runtime as a
function of CPU/GPU workers.\\
Evolution strategies (ES) are a class of black box optimization algorithms inspired by natural
evolution in which at every iteration (generation), a population of parameter vectors (genomes) is
perturbed (mutated) and, optionally, recombined (merged) via crossover. The fitness of each resultant
offspring is then evaluated according to some objective function (reward) and some form of selection
then ensures that individuals with higher reward tend to produce offspring for the next generation.
In openAI's work, a fitness function f($\theta$) represents the stochastic reward experienced over a full episode of agent interaction, where $\theta$ parametrizes the policy $\pi_\theta$.


==> sections/draft/fundamentals_ES.tex <==
\subsection{Main principles behind Evolution Strategies}

\noindent \textit{\remark{Evolution Strategies are a black-box optimization algorithms that search by manipulating the input:-}} Evolution Strategies (ES) is a type of black-box optimization algorithms, derived from Evolutionary Algorithms (EA). Black-box optimization relates to having an objective function which analytical expression  and gradient are unavailable\remark{cite}. The search space is defined as the continuous domain $R^n$, and the objective function will thus be evaluated for each x (representing the n-dimentional solution vectors in the search space) \cite{Zhenhua2020,hansen2015}.
%
Evolution Strategy is therefore a kind of Evolutionary Algorithm rooted in the concept of biological evolution. It is "based on the application of mutation, recombination and selection in populations of candidate solutions" \cite{hansen2015}. It focuses on evaluating the objective function at different points and changing the latter randomly, rather than computing the gradients. \\

\noindent \textit{\remark{A generic evolutionary strategy algorithm:-}}
 The evolution strategy landscape is given in Figure \ref{fig3}. The first step consists of generating a random population P of individuals. Each individual consists of a solution and an associated fitness value, $f(x)$, and can be denoted as a parent individual. There are a total of $\mu$ parents. When in the recombination step, $\lambda$ pairs of these parent individuals are chosen and their respective values are recombined to produce $\lambda$  offspring individuals.This is done by either taking average values or by exchanging randomly chosen components of the parent pair.Gaussian noise is then added to the solutions in the mutation step, allowing for stochastic exploration of the design space. The next step consists of evaluating the individuals’ fitnesses $f(x)$, and only the $\mu$ best individuals from the population survive and are chosen as parent individuals for the next generation.This process then continues and repeats until a stop condition is met \cite{Khan2008}.

\begin{figure}[htbp]
\centerline{\includegraphics[width=\columnwidth]{ES.pdf}}
\caption{A generic evolution strategy and Evolution strategies landscape}
\label{fig3}
\end{figure}

Throughout this paper, Evolutionary Strategies are differentiated from Genetic Algorithms. Table \ref{t1} identifies the main differences between GAs and ESs \cite{HoffmeisterB90}.

\begin{table}[htbp]
\caption{Evolution Strategies vs Genetic Algorithms}
\begin{center}
\label{t1}
\begin{tabular}{p{0.4\linewidth} | p{0.4\linewidth}}
 \hline 
 Evolutionary Strategies & Genetic Algorithms \\
 \hline\hline
 Phenotype level of individuals (real-valued representation) & Genotype level of individuals (binary coding) \\ 
  \hline
 Knowledge of the dimension of the objective function (i.e. number of variables) & No knowledge about the properties of the objective function \\
  \hline
 No parameter restrictions apart from machine-dependencies & Parameter space restrictions for decoding purposes  \\
  \hline
 $(\mu,\lambda)$-selection and $(\mu+\lambda)$-selection & Proportional selection and Ranking \\
  \hline
 Mutation serves as the main search operator  & Recombination serves as the main search operator \\ 
   \hline
 Several recombination schemes & Secondary role of mutation  \\
   \hline
 Collective self-learning of strategy parameters& No collective self-learning of parameter settings  \\
 \hline
\end{tabular}
\label{tab1}
\end{center}
\end{table}

\subsection{Common algorithms}
There are various algorithms defined as being evolution strategies. This section will go over the main ones, giving a high level overview of how it works.

The "Covariance Matrix Adaptation Evolution Strategies (CMA-ES)" defined by Hansen et al. \cite{hansen2016cma} is one of the most popular gradient-free optimisation algorithms, and has been the algorithm of choice for many researchers.  CMA-ES is an algorithm that will take the output of each generation and increase or decrease the search space accordingly for the next generation. This is done based on the $\mu$ and $\sigma$ parameters and on the calculated covariance matrix of the parameter space. The latter adaptation allows CMA-ES to optimize the search space by either increasing it when the best solutions are far away, or narrowing it when the best solutions are close by. At each different generation, CMA-ES samples the solutions from the parameters of a multi-variate normal distribution. CMA-ES has one main drawback relating to its performance decrease in case the number of model parameters to solve for is large, as the covariance calculation is $O(N^2)$.

Natural Evolution Strategies (NES) algorithms iteratively update a search distribution by using an estimated gradient on the distribution parameters \cite{Wierstra2014}. The main steps included for NES are:
\begin{itemize}
  \item The parameterized search distribution is used to produce a batch of search points on which the fitness function will be evaluated.
  \item The distribution’s parameters (including strategy parameters) allow the algorithm to adaptively capture the  structure of the fitness function.
  \item From the samples computed, NES estimates a search gradient on the parameters towards higher expected fitness.
  \item NES then performs a gradient ascent step along the natural gradient, renormalizing the update with respect to uncertainty. This will prevent oscillations, premature convergence, and undesired effects from a given parameterization.
  \item The entire process reiterates until a stopping criterion is met. \cite{Wierstra2014}
\end{itemize}

A third identified Evolution Strategy, is OpenAI-ES. In \cite{salimans2017evolution}, Salimans et al. implemented an evolution strategy that is a simplified special case of the NES algorithm outlined earlier. In particular, $\sigma$ is fixed to a constant number, and only the $\mu$ parameter is updated at each generation. Throughout their paper, Salimans et al. proposed a modification of the update rule that is suitable for parallel computation across different worker machines.This new update rule thus consists of holding a large grid of random numbers which have been pre-computed using a fixed seed. Each worker can then reproduce the parameters of every other worker over time, and each worker needs only to communicate a single number, the final fitness result, to all of the other workers, thus limiting the transmission of an entire solution vector a million times at each generation update which may be unfeasible. The latter allows for scaling evolution strategies to thousands or even a million workers located on different machines. 
The paper by Saliman et al. \cite{salimans2017evolution} opened the doors to many researchers for discussing the competitive aspect of ES, its potential improvements and combination with RL algorithms.\\

==> sections/draft/old_ES.tex <==
\subsection{Main principles}
\noindent Evolution Strategies (ES) is a type of black-box optimization algorithms, derived from Evolutionary Algorithms (EA). With black-box optimization algorithms, a target function $f(x):R_{n}\rightarrow R$ can be evaluated without having to know its precise analytic form. ES's original formulation is dependant on the ideas of mutation, recombination and selection in populations of candidate solutions. It thus mimics biological evolution for optimization, focusing only on function evaluations rather than using gradients, rendering it easily parallelizable. It evaluates the function at different points or the population, randomly changing them. 

The evolution strategy landscape is given in Figure \ref{fig3}. The first step consists of generating a random population P of individuals. Each individual consists
of a solution and an associated fitness value,
f(x), and can be denoted as a parent individual with number $\um$. When in the recombination step, $\lambda$ pairs of these parent
individuals are chosen and their respective values are recombined to produce $\lambda$  offspring
individuals.This is done by either taking average values or by exchanging randomly chosen components
of the parent pair.Gaussian noise is then added to the solutions in the mutation step, allowing for stochastic exploration of the design space. The next step consists of evaluating the individuals’ fitnesses $f(x)$, and only the µ best individuals from the population survive and are chosen as parent individuals for the next generation.This process then continues and repeats until the stopping criteria is met.\cite{b1}

\begin{figure}[htbp]
\centerline{\includegraphics[width=3.3in]{ES.pdf}}
\caption{Evolution strategies landscape}
\label{fig3}
\end{figure}


\begin{table}[htbp]
\caption{Evolution Strategies vs Genetic Algorithms}
\begin{center}
\begin{tabular}{l l l}
 \hline 
   & Evolutionary Strategies & Genetic Algorithms \\
 \hline\hline
 Initial Population & Random mutations & Random or seeded \\ 
%  \hline
 Evaluation & Objective function & Fitness function \\
%  \hline
 Selection & Truncation selection & Different methods  \\
%  \hline
 Reproduction & Recombination + Mutation & Crossover + Mutation \\
%  \hline
 Termination & User dependent & User dependent \\ 
 \hline
\end{tabular}
\label{tab1}
\end{center}
\end{table}


\subsection{Introduction to different evolution strategies}
Throughout this section, various Evolution strategy algorithms will be discussed and further detailed. 


% The basic evolution strategy is defined by $\left( \frac{\mu}{\theta}, \lambda \right)$  (µ/ρ, λ)-ES and (µ/ρ+ λ)-ES:
% \begin{itemize}
%   \item µ The number of selected individuals per generation
%   \item ρ The number of parents (selected from µ) involved in recombination (≤ µ)
%   \item λ The number of individuals per generation (population size)
%   \item , Comma Selection : µ parents are selected from the λ individuals
%   \item + Plus Selection : µ parents are selected from the λ individuals + the
% current ρ parents
% \end{itemize}

% \noindent Example: (10/6, 50)-ES\\
% Select the fittest 10 individuals from the 50 individuals of the current
% population, and select 6 random ones from them. Recombine these 6
% parents to generate 50 new offspring

\subsubsection{Simple Evolution Strategy} \hfill\\
The simple Gaussian evolution strategy is the a basic representation, modeling the probability distribution $p_\theta (x)$ over $x$ as a n-dimensional Gaussian distribution, in which $\theta$ tracks  the mean $\mu$ and standard deviation $\sigma$, carrying the knowledge about the best solutions and being iteratively updated across generations: $\mu = (\mu_x, \mu_y)$ and $\sigma = (\sigma_x, \sigma_y)$.\\
The four main steps involved are described below:
\begin{itemize}
  \item Initialize $\theta$=$\theta^{(0)}$ along with a counter t=0 for keeping track of the generation number. $\mu$ is thus set at the origin
  \item Generate the offspring population by sampling from the Gaussian distribution
  \item Get and evaluate the fitness results.
  \item After the fitness results are evaluated, we set $\mu$ to the best solution in the population, and sample the next generation of solutions around this new mean. 
\end{itemize}


\subsubsection{Covariance-Matrix Adaptation Evolution Strategy}\hfill\\
The CMA-ES is a stochastic, or randomized, method for real-parameter optimization of non-linear, non-convex functions. It can be considered as a solution to the shortcomings of the simpler evolution strategy algorithm or genetic algorithms in terms of having a fixed standard deviation thus limiting exploration. The standard deviation may thus need to be increased at times to properly explore the search space, while other times, when a global optima is close by, fine tuning the solution with a fixed standard deviation might be enough. \\
CMA-ES takes the results of each generation and increases or decreases the search space accordingly for the next generation, thus adapting the mean $\mu$ and variance $\sigma$ parameters while calculating the entire covariance matrix of the parameter space. Getting the covariance matrix tracks the pairwise dependencies between the samples in the distribution. The new distribution thus becomes: $\theta=(\mu,\sigma,C)$\\
There are 3 main steps involved in CMA-ES:
\begin{itemize}
  \item Updating the mean:\hfill\\ $\mu^{(t+1)}=\mu^{(t)}+{\sigma_{\mu}}\frac{1}{\lambda}\sum_{i=1}^{\lambda}(x_{i}^{(t+1)}-\mu^{(t)})$ \\
  CMA-ES has a learning rate $\mu \le 1$ to control how fast the mean μ should be updated. Usually it is set to 1.   
  \item Sampling and Controlling the Step Size: \hfill\\
  In the CMA Evolution Strategy, a population of new search points (individuals, offspring) is generated by sampling a multivariate normal distribution. The basic equation for sampling the search points is: \hfill\\
  $x_i^{(t+1)}=\mu^{(t)}+\sigma^{(t)}y_i^{(t+1)}$ where  $y_i^{(t+1)}=\frac{x_i^{(t+1)}-\mu^{(t)}}{\sigma^{(t)}}$
  The parameter $\sigma$ controls the overall scale of the distribution. It is separated from the covariance matrix so that we can change steps faster than the full covariance. A larger step size leads to faster parameter update. In order to evaluate whether the current step size is proper, CMA-ES constructs an evolution path $p_\sigma$ by summing up a consecutive sequence of moving steps
  \item Adapting the Covariance Matrix:\hfill\\
  For the covariance matrix, it can be estimated from scratch using $y_{i}$ of elite samples.\\
  $C_{lambda}^{(t+1)}=\frac{1}{\lambda}\sum_{(i=1)}^{\lambda}y_{i}^{(t+1)}y_{i}^{(t+1)^{T}}$ \\
  The above estimation is only reliable when the selected population is large enough. However, we do want to run fast iteration with a small population of samples in each generation. That’s why CMA-ES invented a more reliable but also more complicated way to update $C$. It involves two independent routes: Rank-min$(\lambda, n)$ update and Rank-one update. 
\end{itemize} 
\begin{figure}[htbp]
\centerline{\includegraphics[width=3.3in]{CMA-ES-algorithm.png}}
\caption{CMA-ES: Covariance matrix adaptation evolution strategies}
\label{fig2}
\end{figure}

\subsubsection{Natural Evolution Strategies}\hfill\\
Natural Evolution Strategies optimizes in a search distribution of parameters and moves the distribution in the direction of high fitness indicated by the natural gradient.
A perceived weakness of the algorithms mentioned so far is that they discard the majority of the solutions and only keep the best solutions. Weak solutions contain information about what not to do, and this is valuable information to calculate a better estimate for the next generation.\\
In this approach, we want to use all of the information from each member of the population, good or bad, for estimating a gradient signal that can move the entire population to a better direction in the next generation.\\
The idea is to maximise the expected value of the fitness score of a sampled solution. If the expected result is good enough, then the best performing member within a sampled population will be even better, so optimising for the expectation might be a sensible approach. Maximising the expected fitness score of a sampled solution is almost the same as maximising the total fitness score of the entire population.\\
Given an objective function $J(\theta)$ parameterized by $\theta$, the ES goal is to find the optimal θ to maximize the objective function value. The fitness associated with one sample is labeled as f(x) and the search distribution over x is parameterized by $\theta$. NES is expected to optimize the parameter $\theta$ to achieve maximum expected fitness: \\
$J(\theta)=E_{x\sim p_{\theta}(x)}[f(x)]=\int_{x}f(x)p_{\theta}(x)dx$\\
where $\theta$ are the parameters of the probability distribution function. For example, if $p_{\theta}(x)$ is a normal distribution, then $\theta$ would be $\mu$ and $\sigma$.
Using the same log-likelihood trick as in the REINFORCE algorithm allows us to calculate the gradient of $J(\theta)$: \\
$\nabla_\theta J (\theta)=E_{x\sim p_{\theta}(x)}[f(x)\nabla_\theta\log p_\theta(x)]$ \\
With this gradient $\nabla_{\theta} J(\theta)$, we can use a learning rate parameter $\alpha$ (such as 0.01) and start optimising the $\theta$ parameters of pdf $p_{\theta}(x)$ so that our sampled solutions will likely get higher fitness scores on the objective function $F$. We can update $\theta$ for the next generation:\\
$\theta\rightarrow \theta+\alpha \nabla_\tetaJ(\theta)$
 \begin{figure}[htbp]
\centerline{\includegraphics[width=3.3in]{NES-algorithm.png}}
\caption{NES: Canonical Natural evolution strategies}
\label{fig2}
\end{figure}

\subsubsection{OpenAI Evolution Strategy}\hfill\\
In OpenAI’s paper, they implement an evolution strategy that belongs to the class of natural evolution strategies (NES) outlined earlier. In particular, $\sigma$ is fixed to a constant number, and only the $\mu$ parameter is updated at each generation.\\
Researchers at OpenAI thus proposed to use NES as a gradient-free black-box optimizer to find optimal policy parameters $\theta$ that maximizes the return function $F(\theta)$. This is done by adding Gaussian noise $\epsilon$ on the model parameter $\theta$ and then using the log-likelihood method to write it as the gradient of the Gaussian pdf. 
The search distribution of θ is designed to be an isotropic multivariate Gaussian. The gradient for θ update is thus:\\
$\nabla_\theta E _{\in\simN(0,I)}F(\theta+\sigma\in)=\fract{1}{\sigma}E_{\in\simN(0,I)}{F(\theta+\sigma\in)\in}$\\
The resulting algorithm repeatedly executes two phases:
\begin{itemize}
  \item Stochastically perturbing the parameters of the policy and evaluating the resulting parameters by running an episode in the environment
  \item Combining the results of these episodes, calculating a stochastic gradient estimate, and updating the parameters
\end{itemize} 
In addition to the simplification, this paper also proposed a modification of the update rule that is suitable for parallel computation across different worker machines. In their update rule, a large grid of random numbers have been pre-computed using a fixed seed. By doing this, each worker can reproduce the parameters of every other worker over time, and each worker needs only to communicate a single number, the final fitness result, to all of the other workers.

 \begin{figure}[htbp]
\centerline{\includegraphics[width=3.3in]{images/ES-algorithm1.PNG}}
\caption{Evolution strategies}
\label{fig2}
\end{figure}

 \begin{figure}[htbp]
\centerline{\includegraphics[width=3.3in]{images/OpenAI-ES-algorithm.png}}
\caption{Parallelized evolution strategies}
\label{fig2}
\end{figure}

\subsection{Improving on ES}
In the paper "Rapidly Adaptable Legged Robots via Evolutionary Meta-Learning" the authors combine Evolution strategies with meta learning. The latter learns to solve an incoming task quickly without completely retraining from scratch, by combining past experiences with small amounts of experience from the incoming task. It leverages previous experience to explicitly train a policy to be adaptable, by training across many different tasks or environment conditions, allowing for learning new concepts and skills fast with a few training examples. However, applying these techniques to real robots is challenging due to the noise present in real world environments: different initial conditions, hardware wear-and-tear, observation noise, and action noise make exact repetition of trials difficult. The ES-MAML (ES- model-agnostic meta-learning) framework adopted leverages ES for high-dimensional optimization, updating policy based solely on the sum of rewards collected by the agent in the environment. ES thus allows robots to adapt to dynamic changes in the real world, and it is the first instance of successfully using ES for on-robot adaptation.

The paper "Improving Exploration in Evolution Strategies for Deep Reinforcement Learning via a Population of Novelty-Seeking Agents" complements the “Evolution Strategies as a Scalable Alternative to Reinforcement Learning” paper as it aims to show that what would have been considered a shortcoming of ES could actually be fixed by various algorithms ( ES (as well as RL) often ends up converging towards a local maxima). However, algorithms such as novelty search (NS) and quality diversity (QD) can be leveraged with ES to improve its performance on sparse or deceptive deep RL tasks, while retaining scalability, thus encouraging exploration.
Based on the experimentation done throughout the paper, NS-ES and two QD algorithms, NSR-ES and
NSRA-ES avoid local optima encountered by ES to achieve higher performance on Atari and simulated robots learning to walk around a deceptive trap.
Edoardo et al. thus propose throughout this paper different methods for augmenting ES allowing it to perform direct exploration, taking advantage of its scalability while ensuring a higher performance for domains with more sparse reward functions or that appear to have local optima. This opens the way for further similar discussions for RL algorithms.




ES are nature-inspired optimization methods which use random mutation, recombination, and selection applied to a population of individuals containing candidate solutions in order to evolve iteratively better solutions. It is really useful for non-linear or non-convex continuous optimization problems.
In ES, we don’t care much about the function and its relationship with the inputs or parameters. Some million numbers (parameters of the model) go into the algorithm and it spits out 1 value (e.g. loss in supervised setting; reward in case of Reinforcement Learning). We try to find the best set of such numbers which returns good values for our optimization problem. We are optimizing a function J(θ) with respect to the parameters θ, just by evaluating it without making any assumptions about the structure of J, and hence the name ‘black-box optimization’. Let’s dig deep into the implementation details!

